Models for Capturing Temporal Smoothness in Evolving Networks for Learning Latent Representation of Nodes

In a dynamic network, the neighborhood of the vertices evolve across different temporal snapshots of the network. Accurate modeling of this temporal evolution can help solve complex tasks involving real-life social and interaction networks. However, existing models for learning latent representation are inadequate for obtaining the representation vectors of the vertices for different time-stamps of a dynamic network in a meaningful way. In this paper, we propose latent representation learning models for dynamic networks which overcome the above limitation by considering two different kinds of temporal smoothness: (i) retrofitted, and (ii) linear transformation. The retrofitted model tracks the representation vector of a vertex over time, facilitating vertex-based temporal analysis of a network. On the other hand, linear transformation based model provides a smooth transition operator which maps the representation vectors of all vertices from one temporal snapshot to the next (unobserved) snapshot-this facilitates prediction of the state of a network in a future time-stamp. We validate the performance of our proposed models by employing them for solving the temporal link prediction task. Experiments on 9 real-life networks from various domains validate that the proposed models are significantly better than the existing models for predicting the dynamics of an evolving network.

==> expresult.tex <==
%\subsection{Results on Link Prediction Task}
\begin{table*} [!ht]
\begin{subtable}{1.0\linewidth}
\centering
%\ra{0.9}
\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
\begin{tabular}{llll|llll}
\toprule
	\multicolumn{4}{c}{DBLP2} & \multicolumn{4}{c}{DBLP3} \\ 
{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd  & Method & {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
BCGD & 0.7932 $\pm$ 0.03 & 0.8023 $\pm$ 0.03 & 0.8686 $\pm$ 0.02 & BCGD & 0.8564 $\pm$ 0.01 & 0.8599 $\pm$ 0.02 & 0.9524 $\pm$ 0.02 \\
RET (tsvd) & \textbf{0.8360 $\pm$ 0.02} & \textbf{0.8571 $\pm$ 0.01} & \textbf{0.9317 $\pm$ 0.02} & RET (LLE) & \textbf{0.8898 $\pm$ 0.01} & \textbf{0.8926 $\pm$ 0.01} & \textbf{0.9776 $\pm$ 0.01} \\ 
HomoLT (DeepWalk) & 0.7422 $\pm$ 0.03 & 0.7691 $\pm$ 0.04 & 0.8496 $\pm$ 0.05 & HomoLT (LINE) & 0.7557 $\pm$ 0.02 & 0.7818 $\pm$ 0.02 & 0.9671 $\pm$ 0.01 \\
HeterLT (DeepWalk, avg) & 0.7413 $\pm$ 0.02 & 0.7798 $\pm$ 0.02 & 0.8662 $\pm$ 0.02 & HeterLT (LINE, linear) & 0.8301 $\pm$ 0.01 & 0.8680 $\pm$ 0.007 & 0.9934 $\pm$ 0.004 \\
%RET (tsvd) & 0.8360 $\pm$ 0.02 & \textbf{0.8571 $\pm$ 0.01} & \textbf{0.9317 $\pm$ 0.02} & RET (tsvd) & 0.8074 $\pm$ 0.04 & 0.8245 $\pm$ 0.03 & 0.9503 $\pm$ 0.02  \\
%RET (LLE) & \textbf{0.8368 $\pm$ 0.03} & 0.8453 $\pm$ 0.03 & 0.8967 $\pm$ 0.03 & RET (LLE) & \textbf{0.8898 $\pm$ 0.01} & \textbf{0.8926 $\pm$ 0.01} & \textbf{0.9776 $\pm$ 0.01} \\
%RET (ISOMAP) & 0.8187 $\pm$ 0.02 & 0.8346 $\pm$ 0.01 & 0.9098 $\pm$ 0.02 & RET (ISOMAP) & 0.8154 $\pm$ 0.03 & 0.8275 $\pm$ 0.02 & 0.9605 $\pm$ 0.02 \\
%\midrule
\bottomrule
\end{tabular}
}
%\vspace{0.1in}
\caption{DBLP2 and DBLP3}
\label{tab:result-citation1}
\end{subtable}

\begin{subtable}{1.0\linewidth}
\centering
%\ra{1.0}
\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
\begin{tabular}{llll |llll}
\toprule
\multicolumn{4}{c}{HepPH} &\multicolumn{4}{c}{NIPS} \\
{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd & {Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
BCGD                & 0.5732 $\pm$ 0.003 & 0.6170 $\pm$ 0.003 & 0.5542 $\pm$ 0.02 & BCGD	& 0.5157 $\pm$ 0.002	& 0.5457 $\pm$ 0.02 &	0.6118 $\pm$ 0.02 \\
RET (LINE)     & 0.5677 $\pm$ 0.004 & 0.5782 $\pm$ 0.003  & 0.8659 $\pm$ 0.04 & RET (LLE) &	0.5427 $\pm$ 0.04	& 0.5542	$\pm$ 0.02 &  0.5988 $\pm$ 0.08 \\
HomoLT (DeepWalk) & 0.5889 $\pm$ 0.003 &  0.6269 $\pm$ 0.005 & 0.8376 $\pm$ 0.04 & HomoLT (Node2Vec) & \textbf{0.5633 $\pm$ 0.01} & \textbf{0.6123 $\pm$ 0.01} & 0.7947 $\pm$ 0.02 \\
HeterLT (DeepWalk, avg)& \textbf{0.6058 $\pm$ 0.02} & \textbf{0.6346 $\pm$ 0.02} &\textbf{0.9300$\pm$ 0.03} & HeterLT (Node2Vec, wct)  & 0.5581 $\pm$ 0.01 & 0.6211 $\pm$ 0.01 & \textbf{0.8072 $\pm$ 0.03} \\
%RET (DeepWalk) & 0.5679 $\pm$ 0.004 & 0.5818 $\pm$ 0.005  & 0.8623 $\pm$ 0.04  & RET (DeepWalk) & 	0.8382 $\pm$ 0.06 & 	0.8312 $\pm$ 0.07 & 	0.9585 $\pm$ 0.02\\
%RET (LINE)     & 0.5677 $\pm$ 0.004 & 0.5782 $\pm$ 0.003  & \textbf{0.8659 $\pm$ 0.04} & RET (LINE)     &	0.6949 $\pm$ 0.005	&  0.7176 $\pm$ 0.002 & 0.9887 $\pm$ 0.02  \\
%				&     				 & 					   & 					&		RET (Node2Vec) &	\textbf{0.859 $\pm$ 0.004}	& \textbf{0.859	$\pm$ 0.005} &  \textbf{0.9817 $\pm$ 0.006} \\		 
\bottomrule
\end{tabular}
}
%\vspace{0.1in}
\caption{HepPH and NIPS}
\label{tab:tab2}
\end{subtable}

\begin{subtable}{1.0\linewidth}
\centering
\resizebox{0.95\linewidth}{!}{%
\setlength\tabcolsep{8pt}
\begin{tabular}{llll|llll}
\toprule
\multicolumn{4}{c}{Email-EU} &\multicolumn{4}{c}{CollegeMsg} \\
{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd & {Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
BCGD                 & 0.6215 $\pm$ 0.01 & 0.5946 $\pm$ 0.02 & 0.6154 $\pm$ 0.13 & BCGD                & 0.6663 $\pm$ 0.01 &  0.6691 $\pm$ 0.02 &  0.7266 $\pm$ 0.06 \\
RET (LINE)  & 0.9049 $\pm$ 0.005 &  0.9009 $\pm$ 0.009 & 0.9725 $\pm$ 0.02 & RET (PCA) & 0.6291 $\pm$ 0.01 & 0.6435 $\pm$ 0.02 & 0.8381 $\pm$ 0.06 \\ 
HomoLT (LINE)  & 0.8789 $\pm$ 0.009  & 0.8694 $\pm$ 0.01 & 0.9705 $\pm$ 0.01 & HomoLT (LINE) &  {0.7460 $\pm$ 0.01} & {0.7788  $\pm$ 0.01}  &  {0.9571 $\pm$ 0.01} \\
HeterLT(LINE, wct)  & \textbf{0.9211 $\pm$ 0.008} & \textbf{0.9283 $\pm$ 0.006} & \textbf{0.9923 $\pm$ 0.008} & HeterLT (LINE, wct)    &  \textbf{0.7517 $\pm$ 0.01} &  \textbf{0.7913 $\pm$ 0.008}  & \textbf{0.9685 $\pm$ 0.01} \\
%RET (Deepwalk) & 0.7743 $\pm$ 0.01 & 0.7883 $\pm$ 0.02 & 0.9914 $\pm$ 0.01  & HomoL (LINE) &  {0.7460 $\pm$ 0.01} & {0.7788  $\pm$ 0.01}  &  {0.9571 $\pm$ 0.01} \\
%RET (LINE)    & 0.6743 $\pm$ 0.07 & 0.7112 $\pm$ 0.07 & 0.9995  $\pm$ 0.001 & HeterL (LINE, avg)    & 0.7459 $\pm$ 0.02 &  0.7805 $\pm$ 0.01  & 0.9527 $\pm$ 0.02 \\
%RET (Node2Vec)  & \textbf{0.7737 $\pm$ 0.007} & \textbf{0.8089 $\pm$ 0.006} & \textbf{1.0000 $\pm$ 0.00} & HeterLT (LINE, linear)    & 0.7426 $\pm$ 0.02 & 0.7859 $\pm$ 0.01  &  0.9685 $\pm$ 0.01 \\
% & & &  & HeterLT (Line, exp)    &  0.7259 $\pm$ 0.01 &  0.7760 $\pm$ 0.01  & 0.9641 $\pm$ 0.01 \\ 
% & & &	& HeterLT (Line, wct)    &  \textbf{0.7517 $\pm$ 0.01} &  \textbf{0.7913 $\pm$ 0.008}  & \textbf{0.9685 $\pm$ 0.01} \\
\bottomrule
\end{tabular}
}
%\vspace{0.1in}
\caption{Email-EU and CollegeMsg}
\label{tab:tab3}
\end{subtable}

\begin{subtable} {1.0\linewidth}
\centering
%\ra{1.0}
\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
\begin{tabular}{llll|llll}
\toprule
\multicolumn{4}{c}{SMS-A} &\multicolumn{4}{c}{SMS-A} \\
{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd  & {Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
BCGD                & 0.7350 $\pm$ 0.003 &  0.7770 $\pm$ 0.003 &  0.9312 $\pm$ 0.01  & HomoLT (DeepWalk) & 0.6306 $\pm$ 0.005 & 0.6861 $\pm$ 0.006 & 0.9850 $\pm$ 0.01 \\
RET (Node2Vec)         & \textbf{0.7737 $\pm$ 0.007} &  \textbf{0.8089 $\pm$ 0.006}  &  \textbf{1.00 $\pm$ 0.00} & HeterLT (DeepWalk, avg)  & 0.6413 $\pm$ 0.03 & 0.6969 $\pm$ 0.02 & 0.99 $\pm$ 0.03 \\
%HomoLT (LINE) &  0.8789 $\pm$ 0.009 & 0.8694  $\pm$ 0.01  &  0.9705 $\pm$ 0.01 & HomoLT (DeepWalk) & 0.7252 $\pm$ 0.02  & 0.7144 $\pm$ 0.02 & 0.8422 $\pm$ 0.03 \\
%HeterLT (Line, wct)    &  \textbf{0.9211 $\pm$ 0.008} &  \textbf{0.9283 $\pm$ 0.006}  & 0.9923 $\pm$ 0.008 & HeterLT (Node2Vec, linear) & 0.7792 $\pm$ 0.01 & 0.7788 $\pm$ 0.01 & 0.9200 $\pm$ 0.01 \\
%HomoLT (LINE) &  0.8789 $\pm$ 0.009 & 0.8694  $\pm$ 0.01  &  0.9705 $\pm$ 0.01 & RET (LINE) & 0.7871 $\pm$ 0.02 & 0.7882 $\pm$ 0.02 & 0.9445 $\pm$ 0.02 \\
%HeterLT (Line, avg)    & 0.8806 $\pm$ 0.008 &  0.8693 $\pm$ 0.008  & 0.9784 $\pm$ 0.01 &   HeterLT (Node2Vec, avg) & 0.7176 $\pm$ 0.01 & 0.7028 $\pm$ 0.02 & 0.8157 $\pm$ 0.07  \\
%HeterLT (Line, linear)    & 0.9175 $\pm$ 0.006 & 0.9262 $\pm$ 0.004  &  \textbf{0.9933 $\pm$ 0.006} & HeterLT (Node2Vec, linear) & 0.7792 $\pm$ 0.01 & 0.7788 $\pm$ 0.01 & 0.9200 $\pm$ 0.01\\
%HeterLT (Line, exp)    &  0.9177 $\pm$ 0.006 &  0.9262 $\pm$ 0.005  & 0.9909 $\pm$ 0.009 &  HeterLT (Node2Vec, exp) & 0.7698 $\pm$ 0.01 & 0.7667 $\pm$ 0.01 & 0.9037 $\pm$ 0.01 \\
%HeterLT (Line, wct)    &  \textbf{0.9211 $\pm$ 0.008} &  \textbf{0.9283 $\pm$ 0.006}  & 0.9923 $\pm$ 0.008 & HeterLT (Node2Vec, wct) & 0.7712 $\pm$ 0.01 & 0.7671 $\pm$ 0.01 & 0.8956 $\pm$ 0.01  \\
\bottomrule
\end{tabular}
}
%\vspace{0.1in}
\caption{SMS-A}
\label{tab:tab4}
\end{subtable}

\begin{subtable}{1.0\linewidth}
\centering
%\ra{1.0}
\resizebox{0.95\linewidth}{!}{%
\setlength\tabcolsep{8pt}
\begin{tabular}{llll| llll}
\toprule
\multicolumn{4}{c}{Facebook} &\multicolumn{4}{c}{Facebook2} \\
{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd & {Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
BCGD & 0.6431 $\pm$ 0.002 & 0.6576 $\pm$ 0.003 & 0.3694 $\pm$ 0.02  & BCGD & 0.7537 $\pm$ 0.02 & 0.7190 $\pm$ 0.02  & 0.7957 $\pm$ 0.05 \\
RET (Node2Vec) & \textbf{0.859 $\pm$ 0.004} & \textbf{0.859 $\pm$ 0.005} & 0.9817 $\pm$ 0.006 & RET(PCA) & \textbf{0.8202 $\pm$ 0.01} & \textbf{0.8144 $\pm$ 0.01} & \textbf{0.9519 $\pm$ 0.02} \\
HomoLT (DeepWalk) & 0.6061 $\pm$ 0.004 & 0.6141 $\pm$ 0.004 & 0.7113 $\pm$ 0.02 & HomoLT (DeepWalk) & 0.7252 $\pm$ 0.02 &0.7144 $\pm$ 0.02  & 0.8422 $\pm$ 0.03\\
HeterLT (LINE, avg)  & 0.6258 $\pm$ 0.02 & 0.6983 $\pm$ 0.02 & \textbf{0.9823 $\pm$ 0.03} & HeterLT (Node2Vec, linear) & 0.7792 $\pm$ 0.01 & 0.7788 $\pm$ 0.01 & 0.9200 $\pm$ 0.01\\
%HomoLT (PCA) & 0.5446 $\pm$ 0.007 & 0.5510 $\pm$ 0.007 & 0.9421 $\pm$ 0.02 & & & &  \\
%HeterLT (Node2Vec, avg) & 0.5557 $\pm$ 0.01 & 0.6191 $\pm$ 0.01 & 0.8013 $\pm$ 0.03  & HeterLT (PCA, avg) & 0.5340 $\pm$ 0.01 & 0.5412 $\pm$ 0.01 & 0.9439 $\pm$ 0.03 \\
%HeterLT (Node2Vec, linear) & 0.5641 $\pm$ 0.02 & 0.6233 $\pm$ 0.02 & 0.7952 $\pm$ 0.04 & HeterLT (PCA, linear) & 0.5393 $\pm$ 0.009 & 0.5465 $\pm$ 0.007 & 0.9563 $\pm$ 0.02 \\
%HeterLT (Node2Vec, exp) & 0.5622 $\pm$ 0.01 & 0.6192 $\pm$ 0.02 & 0.7849 $\pm$ 0.04 & HeterLT (PCA, exp) & 0.5409 $\pm$ 0.009 & 0.5472 $\pm$ 0.007 & 0.9539 $\pm$ 0.02 \\
%HeterLT (Node2Vec, wct) & \textbf{0.5581 $\pm$ 0.01} & \textbf{0.6211 $\pm$ 0.01} & 0.8072 $\pm$ 0.03 & HeterLT (PCA, wct) & 0.5460 $\pm$ 0.008 & 0.5514 $\pm$ 0.006 & \textbf{0.9626 $\pm$ 0.01}  \\
%\midrule
\bottomrule
\end{tabular}
}
\caption{Facebook and Facebook2}
\label{tab:tab5}
\end{subtable}
%\vspace{-0.1in}
\caption{Performance of seven of our Homogeneous models, 28 of our Heterogeneous models, and 7 of our retrofitted models, on nine datasets. The highlighted results are statistically significant over the baseline with p<0.001. For fair comparison, we set the latent dimension size to 64. }
\label{tab:all}
\end{table*}


%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline
%BCGD & 0.7537 $\pm$ 0.02 & 0.7190 $\pm$ 0.02 & 0.7957 $\pm$ 0.05 \\\hline 
%RET (PCA)  & 0.8202 $\pm$ 0.01 & 0.8144 $\pm$ 0.01 & 0.9519 $\pm$ 0.02  \\
%RET (LINE) & 0.7871 $\pm$ 0.02 & 0.7882 $\pm$ 0.02 & 0.9445 $\pm$ 0.02  \\\hline 
%HeterLT (Node2Vec, avg) & 0.7176 $\pm$ 0.01 & 0.7028 $\pm$ 0.02 & 0.8157 $\pm$ 0.07 \\
%HeterLT (Node2Vec, linear) & 0.7792 $\pm$ 0.01 & 0.7788 $\pm$ 0.01 & 0.9200 $\pm$ 0.01 \\
%HeterLT (Node2Vec, exp) & 0.7698 $\pm$ 0.01 & 0.7667 $\pm$ 0.01 & 0.9037 $\pm$ 0.01 \\
%HeterLT (Node2Vec, wct) & 0.7712 $\pm$ 0.01 & 0.7671 $\pm$ 0.01 & 0.8956 $\pm$ 0.01 \\
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{Facebook2 (64) Results}
%\label{tab:social2}
%\end{table}

%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
%BCGD & 0.5157 $\pm$ 0.02 & 0.5457 $\pm$ 0.02 & 0.6118 $\pm$ 0.02  \\\hline
%HomoLT (Node2Vec) & 0.5633 $\pm$ 0.01 & 0.6123 $\pm$ 0.01 & 0.7947 $\pm$ 0.02 \\
%HomoLT (PCA) & 0.5446 $\pm$ 0.007 & 0.5510 $\pm$ 0.007 & 0.9421 $\pm$ 0.02 \\\hline 
%HeterLT (Node2Vec, avg) & 0.5557 $\pm$ 0.01 & 0.6191 $\pm$ 0.01 & 0.8013 $\pm$ 0.03 \\
%HeterLT (PCA, avg) & 0.5340 $\pm$ 0.01 & 0.5412 $\pm$ 0.01 & 0.9439 $\pm$ 0.03 \\ \hline
%HeterLT (Node2Vec, linear) & 0.5641 $\pm$ 0.02 & 0.6233 $\pm$ 0.02 & 0.7952 $\pm$ 0.04 \\
%HeterLT (PCA, linear) & 0.5393 $\pm$ 0.009 & 0.5465 $\pm$ 0.007 & 0.9563 $\pm$ 0.02 \\ \hline
%HeterLT (Node2Vec, exp) & 0.5622 $\pm$ 0.01 & 0.6192 $\pm$ 0.02 & 0.7849 $\pm$ 0.04 \\
%HeterLT (PCA, exp) & 0.5409 $\pm$ 0.009 & 0.5472 $\pm$ 0.007 & 0.9539 $\pm$ 0.02 \\\hline
%HeterLT (Node2Vec, wct) & 0.5581 $\pm$ 0.01 & 0.6211 $\pm$ 0.01 & 0.8072 $\pm$ 0.03 \\
%HeterLT (PCA, wct) & 0.5460 $\pm$ 0.008 & 0.5514 $\pm$ 0.006 & 0.9626 $\pm$ 0.01 \\
%\midrule
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{NIPS (64) Results}
%\label{tab:result-citation2}
%\end{table}


%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
%BCGD                & 0.5732 $\pm$ 0.003 & 0.6170 $\pm$ 0.003 & 0.5542 $\pm$ 0.02 \\
%RET (DeepWalk) & 0.5679 $\pm$ 0.004 & 0.5818 $\pm$ 0.005  & 0.8623 $\pm$ 0.04 \\
%RET (LINE)     & 0.5677 $\pm$ 0.004 & 0.5782 $\pm$ 0.003  & 0.8659 $\pm$ 0.04 \\
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{HepPH (64) Results}
%\label{tab:result-citation3}
%\end{table}

In Table~\ref{tab:all}, we show the comparison between the competing method (BCGD) and
our proposed models: retrofitting (RET), homogeneous transformation (HomoLT),
and heterogeneous transformation (HeterLT). 
Our models' performances vary for each base embedding method they implement. Therefore, we only report the results from the best-performing base embedding model (name in parentheses).
In cases where the best-performing base models differ for different metrics, we present the results of the base model that is best overall, in boldface font.

Table~\ref{tab:all}. shows that one of our three proposed methods outperforms BCGD in all three metrics over all datasets.
This suggests that the latent embedding vectors from our proposed models
are better for link prediction than BCGD's embedding vectors.

A possible explanation for BCGD's underperformance is that because BCGD 
We think BCGD may underperform because it can only exploits edge-based proximity when learning latent embedding vectors by factoring the adjacency matrix. Whereas, our
models capture more complex network proximity by implementing, as base embedding models, state-of-the-art static node embedding methods.
%One possible explanation is that BCGD factors the adjacency matrix, so the latent embedding vectors that are learned using BCGD reflect only the edge based proximity whereas our models use state-of-the-art static node embedding methods as base embedding models, which capture more complex network proximity. 

%Also, our local and global temporal smoothness methods provide a better dynamic network model than the one that is proposed in BCGD. Below, We present the results in details by grouping them over the three different kinds of networks. 

\subsection{Link Prediction in Citation Network}
Results of three collaboration networks are given in Table~\ref{tab:result-citation1} and ~\ref{tab:tab2}.
Among the citation networks, DBLP2 and DBLP3 results are similar (see Table ~\ref{tab:result-citation1}); for both the datasets the
retrofitted model (RET) performs the best in all three metrics; For DBLP2, RET improves
the AUC, PRAUC, and NDCG values of the competing BCGD method by 0.04, 0.06, and 0.06 units, which translates to 
5\%, 7\%, and 7\% improvement, respectively. For DBLP3, the improvement of RET on these three
metrics are 0.04, 0.03, and 0.02. Interestingly, the base learning models of the best performing
RET differs over these datasets, for DBLP2, it is tsvd and for DBLP3, it is LLE. The performance
of HomoLT and HeterLT in comparison to BCGD are mixed over different metrics. For instance, 
they are better in NDCG metric, but marginally worse in the AUC, and PRAUC metrics. 

For the NIPS dataset (see Table \ref{tab:tab2}), the transformation models (HomoLT and HeterLT) are the
best performing models. Homogeneous and Heterogeneous models with Node2Vec as the base embedding model
have the best performance; HomoLT is the winner in AUC and PRAUC, and HeterLT is the winner in NDCG.
In fact, the NDCG value of HeterLT is .8072, which is better than the same for BCGD by 0.19 unit, more than
30\% improvement! For AUC metric, the improvement is around 0.04 unit and for PRAUC metric the improvement
is around 0.06 unit for both the homogeneous and heterogeneous models. 
In NIPS dataset, RTE model has a mixed performance compared to BCGD, the former wins in AUC and PRAUC, but loses in NDCG, both marginally.
An explanation of sub-optimal performance by the retrofitted model in this dataset may come from its large number of time snapshots (17); due to
this reason, the vectors of last time snapshot, which are obtained by 16 iterations of retrofitting of the base embedding vectors of first snapshot, 
may wandered away from their optimal position. Another explanation is that in this dataset the number of unique edges (4733) is quite close to the number
of total interaction (5461); i.e., edges are not repeated so each new snapshot is very different than the previous snapshots and retrofitting may not
the ideal approach for capturing the temporal smoothness of this dataset. HepPH dataset also have same behavior as NIPS (results are available in the same table). In this dataset the best
performing model is HeterLT with Deepwalk as the base embedding. In fact HeterLT has more than 30\% improvement over the BCGD model in NDCG metric, and
around 5\% improvement in two other metrics. For this dataset also RET has mixed performance with respect to BCGD. The suboptimal performance of retrofitting
models may be due to the very small ratio of the number of distinct edges and the total number of interactions.

%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
%BCGD                & 0.6215 $\pm$ 0.01 &  0.5946 $\pm$ 0.02 &  0.6154 $\pm$ 0.13 \\
%RET (LINE)         & 0.9049 $\pm$ 0.005 &  0.9009 $\pm$ 0.009 &  0.9725 $\pm$ 0.02 \\
%HomoL (LINE) &  0.8789 $\pm$ 0.009 & 0.8694  $\pm$ 0.01  &  0.9705 $\pm$ 0.01 \\
%HeterL (Line, avg)    & 0.8806 $\pm$ 0.008 &  0.8693 $\pm$ 0.008  & 0.9784 $\pm$ 0.01 \\
%HeterL (Line, linear)    & 0.9175 $\pm$ 0.006 & 0.9262 $\pm$ 0.004  &  0.9933 $\pm$ 0.006 \\
%HeterL (Line, exp)    &  0.9177 $\pm$ 0.006 &  0.9262 $\pm$ 0.005  & 0.9909 $\pm$ 0.009 \\
%HeterL (Line, wct)    &  0.9211 $\pm$ 0.008 &  0.9283 $\pm$ 0.006  & 0.9923 $\pm$ 0.008 \\
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{Email-EU (64) Results}
%\label{tab:result-messaging1}
%\end{table}


%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
%BCGD                 & 0.7350 $\pm$ 0.003 & 0.7770 $\pm$ 0.003 & 0.9312 $\pm$ 0.01 \\
%RET (deepwalk) & 0.7743 $\pm$ 0.01 & 0.7883 $\pm$ 0.02 & 0.9914 $\pm$ 0.01 \\
%RET (LINE)    & 0.6743 $\pm$ 0.07 & 0.7112 $\pm$ 0.07 & 0.9995  $\pm$ 0.001\\
%RET (Node2Vec)  & 0.7737 $\pm$ 0.007 & 0.8089 $\pm$ 0.006 & 1.0000 $\pm$ 0.00\\
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{SMS-A (64) Results}
%\label{tab:result-messaging2}
%\end{table}


%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
%BCGD                & 0.6663 $\pm$ 0.01 &  0.6691 $\pm$ 0.02 &  0.7266 $\pm$ 0.06 \\
%HomoL (LINE) &  0.7460 $\pm$ 0.01 & 0.7788  $\pm$ 0.01  &  0.9571 $\pm$ 0.01 \\
%HeterL (Line, avg)    & 0.7459 $\pm$ 0.02 &  0.7805 $\pm$ 0.01  & 0.9527 $\pm$ 0.02 \\
%HeterL (Line, linear)    & 0.7426 $\pm$ 0.02 & 0.7859 $\pm$ 0.01  &  0.9685 $\pm$ 0.01 \\
%HeterL (Line, exp)    &  0.7259 $\pm$ 0.01 &  0.7760 $\pm$ 0.01  & 0.9641 $\pm$ 0.01 \\
%HeterL (Line, wct)    &  0.7517 $\pm$ 0.01 &  0.7913 $\pm$ 0.008  & 0.9685 $\pm$ 0.01 \\
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{CollegeMsg (64) Results}
%\label{tab:result-messaging3}
%\end{table}


\subsection{Link Prediction in Messaging Network}
The results of the messaging datasets are shown in Table~\ref{tab:tab3} and Table~\ref{tab:tab4}.

For Email-EU, all our proposed methods perform better than the BCGD model in substantial margin; HeterLT (LINE) model performs the best in all three metrics combined. For example, HeterLT (LINE) model improves the NDCG value of BCGD by 0.38 unit, from 0.6154 to 0.9959! Similar large margins can also be seen in other two metrics (please see Table~\ref{tab:tab3} (Left) for the detailed results).
For this dataset retrofitting models also perform substantially better than BCGD. A possible explanation is the high ratio of
distinct edge and the number of interactions, i.e., the earlier edges are repeated in later iterations, so the retrofitting based temporal smoothness of the node vectors are sufficient for capturing the network dynamics
in this dataset. CollegeMsg dataset also has similar behavior with HeterLT (LINE) as the winner among all, again with substantial performance gain (around 20\% to 30\% improvement of performance value across all three
metrics). For this dataset, retrofitting results are poor which could be due to small ratio of distinct edge vs interaction count, and large number of temporal snapshots.
For SMS-A dataset (results is shown on both side of Table~\ref{tab:tab4}), retrofitted
method with Node2Vec as the initial representation generator performs the best. The model achieves 0.04 unit improvement in AUC, 0.03 unit in AUPRC and 0.07 unit in NDCG over BCGD. For this dataset, the ratio of distinct
edge vs interaction count is higher than the CollegeMsg dataset, which could be a reason for the RET model to perform better.

%\begin{table} [!ht]
%\centering
%\ra{1.0}
%\resizebox{0.95\linewidth}{!}{%
%\setlength\tabcolsep{8pt}
%\begin{tabular}{llll}
%\toprule
%{Method}& {AUC $\pm$ sd} & {AUPRC $\pm$ sd} & $NDCG_P$ $\pm$ sd \\\hline 
%BCGD	& 0.6431 $\pm$ 0.0029	& 0.6576 $\pm$ 0.003 &	0.3694 $\pm$ 0.02 \\
%RET (DeepWalk) & 	0.8382 $\pm$ 0.06 & 	0.8312 $\pm$ 0.07 & 	0.9585 $\pm$ 0.02 \\
%RET (LINE)     &	0.6949 $\pm$ 0.005	&  0.7176 $\pm$ 0.002 & 	0.9887 $\pm$ 0.02 \\
%RET (Node2Vec) &	0.859 $\pm$ 0.004	& 0.859	$\pm$ 0.005 &  0.9817 $\pm$ 0.006 \\
%\bottomrule
%\end{tabular}
%}
%\vspace{0.1in}
%\caption{Facebook (32) Results}
%\label{tab:social1}
%\end{table}

\subsection{Link Prediction in Social Network}
Results on social networks are shown in Table~\ref{tab:tab5}.
For Facebook and Facebook2, the retrofitted
method with Node2Vec and PCA performs better than BCGD. RET (Node2Vec) performs the best in Facebook dataset. The model gains 0.21 unit improvement over BCGD in AUC metric, 0.20 unit in AUPRC, and around 0.60 unit in NDCG metric. For Facebook2 dataset, RET (PCA) performs the best. RET (PCA) improves 0.07 unit over BCGD in AUC metric, 0.10 unit in AUPRC metric, and 0.16 unit in the NDCG metric. Heterogeneous method with Node2Vec as the representation generator along with linear or exponential smoothing operator also performs better than BCGD achieving around 0.06 unit improvement in AUPRC, and 0.13 unit improvement in NDCG metric. The Facebook datasets 
have small number of timestamps, which is a likely reason for RET model to perform better than the transformation based models on these datasets.

\begin{figure*}[!ht]\centering
   \centering
	%\hspace{-0.4in}
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[scale=0.42]{figures/dblp2_latent.eps} 
        \caption{DBLP2} \label{fig:a}
    \end{subfigure}
    %\hspace{0.2in}
    \begin{subfigure}{0.33\linewidth}
        \centering
        \includegraphics[scale=0.42]{figures/college_latent.eps} 
        \caption{CollegeMsg} \label{fig:b}
    \end{subfigure}
   %\hspace{0.2in}
   \begin{subfigure}{0.33\linewidth}
       \centering
       \includegraphics[scale=0.42]{figures/fb2_latent.eps} 
       \caption{Facebook2} \label{fig:c}
   \end{subfigure}
\vspace{-0.2in} 
\caption{Effect on Latent Dimension. We evaluate the performance of our best models along with the baseline model to study the effect of different latent dimension (in our case, 32, 64, and 128).}
\label{fig:latentDimension}
\end{figure*}


\subsection{Effect of Latent Dimensions} \label{sec:lat-dim}
In Figure \ref{fig:latentDimension}, we present the performance in NDCG metric of the baseline model (BCGD) along with our best models for three different dataset (one representative dataset from each network group) and over three different latent dimension: 32, 64, and 128. In all three datasets, the performance of multiple of our models is consistently better than BCGD over all three latent dimensions.
BCGD shows marginal improvement as the latent dimension increases. Most of our models stay flat or increases slowly as the dimension size increases because our models already achieve very high NDCG even in the low dimension (at dimension size, 32). The performance of RET (tsvd) and HeterLT (Node2Vec, avg) deceases in DBLP2 and Facebook2, respectively as the dimension size increases from 64 to 128. However, the decrement is only around 2 points in both cases. 

% \subsection{Effect of Non-linearity}
% For this experiment, we keep the base representation model for the Homogeneous and Heterogeneous model fixed (Deepwalk with latent dimension 64) and then introduce three types of non-linearity (Sigmoid, Tanh and Relu). Thereof, we evaluate three different Homogeneous combination and twelve (three non-linearity  $\times$ four different combination of smoothing model) different combination of Heterogeneous models. Please see Section \ref{sec:lp} () for details of the model. We present our findings in the following paragraph. We use four dataset: DBLP2 and DBLP3 from the citation networks, CollegeMsg from Messaging Networks, and Facebook2 from the Social Networks. For all the datasets, we did not see any statistically significant improvement for introducing non-linearity. 


==> fig2.tex <==
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\begin{figure}
\pgfmathsetseed{1}
\begin{tikzpicture}
\definecolorseries{test}{rgb}{step}[rgb]{.95,.85,.55}{.17,.47,.37}
\def\startx{0}
\def\starty{0}

\resetcolorseries[55]{test} 
\newcommand*{\XAxisMin}{0}%
\newcommand*{\XAxisMax}{6}%
\newcommand*{\OriginX}{0}%
\newcommand*{\OriginY}{0.0}%
\newcommand*{\IncrY}{1.0}
\newcommand*{\IncrX}{0.1}
\newcommand*{\Xextension}{6}
\newcommand*{\Yextension}{1}
\newcommand*{\IncrYDM}{0.7}

\def\startxx{0}
\def\startyy{0}


\node () at (\startx - 0.2,\starty+1.4) {\Large $\phi_1$};  
\node () at (\startx + 2.0,\starty+1.4) {\Large $\phi_2$}; 
%\node () at (\startx+7.2,\starty+1.1) {\Large $\phi_2$};  
\node () at (\startx + 4.1,\starty+1.4) {\Large $\phi_3$}; 

\node[draw] () at (\startx + 7.0,\starty+1.4) {\Huge $\phi_4$};

\node () at (\startx - 0.4,\starty+4.5) {\Large $G_1$};  
\node () at (\startx + 2.0,\starty+4.5) {\Large $G_2$};
\node () at (\startx + 4.3,\starty+4.5) {\Large $G_3$};
\node () at (\startx + 6.2,\starty+4.5) {\Large $G_4$};


%\node () at (\startx + 2.2,\starty+1.1) {\Large $\phi_2$}; 
%\node () at (\startx+7.2,\starty+1.1) {\Large $\phi_2$};  
%\node () at (\startx + 4.7,\starty+1.1) {\Large $\phi_3$}; 

\draw[thick, -] (\startxx+5.9,\startyy+0.8) -- (\startxx+5.9,\startyy+4.9);
\draw[thick, -] (\startxx+5.9,\startyy+0.8) -- (\startxx+5.9,\startyy+4.9);


\draw[thick, -] (\startxx,\startyy+2.8) -- (\startxx+7.7,\startyy+2.8);


\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.5,\OriginY+\startyy+4.5) {\Large A};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) {\Large B};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) {\Large E};

\draw[thick,-] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.3) -- (\startxx+0.9,\startyy+3.8);
\draw[thick,-] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.3) -- (\startxx+0.0,\startyy+3.8);

%\draw[thick,->] (\OriginX+\startxx+0.5,\OriginY+\startyy+3.1) -- (\startxx+0.5,\startyy+1.8);
%\draw[thick,->] (\OriginX+\startxx+1.0,\OriginY+\startyy+1.6) -- (\startxx+2.8,\startyy+3.0);

%\draw [fill=none] (\startx+2.1,\starty+2.0) rectangle (\startx+3.0,\starty+2.5) node[pos=.5] {RT};


%\node (a) at (\OriginX+3.0, \OriginY-0.2in) { \Large Problem Definition};
%\node[rotate=45] at (\startxx-0.2,\startyy+2.4) {DeepWalk};
%\node[rotate=45] at (\startxx+2.3,\startyy+2.2) {RET};


\def\startxx{2.2}
\def\startyy{0}

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.5,\OriginY+\startyy+4.5) {\Large A};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) {\Large C};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) {\Large D};

\draw[thick,-] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.3) -- (\startxx+0.9,\startyy+3.8);
\draw[thick,-] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.3) -- (\startxx+0.0,\startyy+3.8);
%\draw[thick,->] (\OriginX+\startxx+0.5,\OriginY+\startyy+3.1) -- (\startxx+0.5,\startyy+1.8);
%\draw[thick,->] (\OriginX+\startxx+1.0,\OriginY+\startyy+1.6) -- (\startxx+2.8,\startyy+3.0);

%\node[rotate=45] at (\startxx+2.3,\startyy+2.2) {RET};

\def\startxx{4.4}
\def\startyy{0}
\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.5,\OriginY+\startyy+4.5) {\Large A};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) {\Large B};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) {\Large E};

\draw[thick,-] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.3) -- (\startxx+0.9,\startyy+3.8);
\draw[thick,-] (\OriginX+\startxx+0.5,\OriginY+\startyy+4.3) -- (\startxx+0.0,\startyy+3.8);
%\draw[thick,->] (\OriginX+\startxx+0.7,\OriginY+\startyy+3.1) -- (\startxx+0.7,\startyy+1.8);

\def\starty{0.7}

\foreach \x in {\startx,\startx+0.5}{
    \foreach \y in {\starty,\starty+0.3,\starty+0.6,\starty+0.9,\starty+1.2}
        \fill[test!!+] (\x,\y) rectangle ++(0.5,0.5);
    }
\foreach \x in {\startx+2.3,\startx+2.8}{
    \foreach \y in {\starty,\starty+0.3, \starty+0.6, \starty+0.9, \starty+1.2}
        \fill[test!!+] (\x,\y) rectangle ++(0.5,0.5);
       }
\foreach \x in {\startx+4.3,\startx+4.8}{
    \foreach \y in {\starty,\starty+0.3, \starty+0.6, \starty+0.9, \starty+1.2}
        \fill[test!!+] (\x,\y) rectangle ++(0.5,0.5);
       }


\def\startxx{6.8}
\def\startyy{0}
\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+1.0,\OriginY+\startyy+4.5) circle (0.3cm) node[] at (\OriginX+\startxx+1.0,\OriginY+\startyy+4.5) {\Large A};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.0,\OriginY+\startyy+4.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.0,\OriginY+\startyy+4.5) {\Large D};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+0.0,\OriginY+\startyy+3.5) {\Large B};

\draw [black,thick, line width=0.5mm] (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) circle (0.3cm) node[] at (\OriginX+\startxx+1.0,\OriginY+\startyy+3.5) {\Large E};

\draw[thick,-] (\OriginX+\startxx+1.0,\OriginY+\startyy+4.3) -- (\startxx+1.0,\startyy+3.8);
\draw[thick,-] (\OriginX+\startxx+1.0,\OriginY+\startyy+4.3) -- (\startxx+0.0,\startyy+3.8);
\draw[thick,-] (\OriginX+\startxx+0.0,\OriginY+\startyy+3.8) -- (\startxx+0.0,\startyy+4.3);


\end{tikzpicture}
\caption{Pictorial depiction of problem definition.}
\label{fig:intro}
\end{figure}

==> ideas.tex <==
1. Can we learn compositionality? i.e. given two nodes, can we learn transformation matrix/tensor to compose two node representation into one?
https://nlp.stanford.edu/~socherr/EMNLP2013_RNTN.pdf


2. Use of Log bilinear model.

3. Using a neural network to model transition from step 1 to t-1 to learn hetergeneous weights and then use exponential averaging to get the final weighting.

==> intro.tex <==
{\blue {Page Limit: 9 Pages\\}}
The underlying
problem can be stated as follows: Given a sequence of graph
snapshots, $\mathbb{G}$ = \{$G_1$, $G_2$, $G_3$, \dots ,$G_t$ \}, how can we infer the temporal latent space so
that at each time point the latent position of a node does not move far way from its previous position? However, compared to the existing work, our objective is little bit different. In this work, we want to exploit the goodness in the existing latent representation techniques to infer the temporal latent space.


This paper is organized as follows: In Section \ref{sec:tempn2v:relwork}, we introduce
the related works about static and dynamic network embedding 
computation, and models for capturing temporal smoothness.

\input{mainfig.tex}

==> mainfig.tex <==
\newcommand*{\XAxisMin}{0}%
\newcommand*{\XAxisMax}{6}%
\newcommand*{\OriginX}{0}%
\newcommand*{\OriginY}{0.0}%
\newcommand*{\IncrY}{1.0}
\newcommand*{\IncrX}{0.1}
\newcommand*{\Xextension}{6}
\newcommand*{\Yextension}{1}
\newcommand*{\IncrYDM}{0.7}

\begin{figure}
\centering
\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
\draw [black,thick, line width=0.5mm] (\OriginX,\OriginY) circle (0.5cm) node[] at (\OriginX,\OriginY) {\Huge A};
\draw [] (\OriginX,\OriginY+2.0) circle (0.5cm) node[] at (\OriginX,\OriginY+2*\IncrY) {\Huge B};

\node (A) at (\OriginX,\OriginY+0.3) {};
\node (B) at (\OriginX,\OriginY+2.0-0.3) {};
\draw [-, line width= 0.3 mm] (A) edge (B);

\draw [black, thick, line width=0.5mm] (\OriginX+2.5,\OriginY) circle (0.5cm) node[] at (\OriginX+2.5,\OriginY) {\Huge A};
%\draw [] (\OriginX+2.0,\OriginY+2.0) circle (0.5cm) node[] at (\OriginX+2.0,\OriginY+2*\IncrY) {\Huge 29};
\draw [] (\OriginX+4.5,\OriginY) circle (0.5cm) node[] at (\OriginX+4.5,\OriginY) {\Huge C};
\draw [] (\OriginX+4.5,\OriginY+2.0) circle (0.5cm) node[] at (\OriginX+4.5,\OriginY+2.0) {\Huge D};

%\node (C) at (\OriginX+2.0,\OriginY+0.3) {};
%\node (D) at (\OriginX+2.0,\OriginY+2.0-0.3) {};
%\draw [-, line width= 0.3 mm] (C) edge (D);

\node (E) at (\OriginX+2.5+ 0.3,\OriginY) {};
\node (F) at (\OriginX+4.5 -0.3,\OriginY) {};
\draw [-, line width= 0.3 mm] (E) edge (F);

\node (G) at (\OriginX+2.3+ 0.3,\OriginY+0.3) {};
\node (H) at (\OriginX+4.5 -0.3,\OriginY+2.0-0.3) {};
\draw [-, line width= 0.3 mm] (G) edge (H);

\draw [thick,dashed, line width= 0.5 mm] (\OriginX+1.8, \OriginY-6.2) -- (\OriginX+1.8, \OriginY+3.0);
\draw [thick,dashed, line width= 0.5 mm] (\OriginX+5.5, \OriginY-6.2) -- (\OriginX+5.5, \OriginY+3.0);

\node (b) at (\OriginX, \OriginY-1.0) {\Huge t=1};
\node (a) at (\OriginX+3.7, \OriginY-1.8) {\Huge (a) };
\node (c) at (\OriginX+3.5, \OriginY-1.0) {\Huge t=2};


\draw [black,thick, line width=0.5mm] (\OriginX+7.0,\OriginY) circle (0.5cm) node[] at (\OriginX+7.0,\OriginY) {\Huge A};
\draw [] (\OriginX+7.0,\OriginY+2.0) circle (0.5cm) node[] at (\OriginX+7.0,\OriginY+2*\IncrY) {\Huge B};

\node (A) at (\OriginX+7.0,\OriginY+0.3) {};
\node (B) at (\OriginX+7.0,\OriginY+2.0-0.3) {};
\draw [-, line width= 0.3 mm] (A) edge (B);

\node (c) at (\OriginX+7.0, \OriginY-1.0) {\Huge t=3};


\draw [thick, ->, line width=0.5mm] (\OriginX-1.0, \OriginY-6.0) -- (\OriginX+10.0, \OriginY-6.0);


\draw [black, line width=0.5mm] (\OriginX-0.5,\OriginY-5.0) circle (0.5cm) node[] at (\OriginX-0.5,\OriginY-5.0) {\Huge A};
\draw [black, line width=0.5mm] (\OriginX-0.5,\OriginY-4.5+0.7) circle (0.5cm) node[] at (\OriginX-0.5,\OriginY+2*\IncrY-5.7) {\Huge B};

\draw [black, line width=0.5mm] (\OriginX+1.2,\OriginY-5.0) circle (0.5cm) node[] at (\OriginX+1.2,\OriginY-5.0) {\Huge C};
\draw [black, line width=0.5mm] (\OriginX+1.2,\OriginY-4.5+1.7) circle (0.5cm) node[] at (\OriginX+1.2,\OriginY+2*\IncrY-4.7) {\Huge D};


\draw [black, line width=0.5mm] (\OriginX+3.5,\OriginY-5.0) circle (0.5cm) node[] at (\OriginX+3.5,\OriginY-5.0) {\Huge A};
\draw [black, line width=0.5mm] (\OriginX+3.0,\OriginY-4.5+0.7) circle (0.5cm) node[] at (\OriginX+3.0,\OriginY+2*\IncrY-5.7) {\Huge B};

\draw [black, line width=0.5mm] (\OriginX+4.5,\OriginY-5.0) circle (0.5cm) node[] at (\OriginX+4.5,\OriginY-5.0) {\Huge C};
\draw [black, line width=0.5mm] (\OriginX+4.5,\OriginY-4.5+1.2) circle (0.5cm) node[] at (\OriginX+4.5,\OriginY-3.3) {\Huge D};


\draw [black, line width=0.5mm] (\OriginX+6.5,\OriginY-5.0) circle (0.5cm) node[] at (\OriginX+6.5,\OriginY-5.0) {\Huge A};
\draw [black, line width=0.5mm] (\OriginX+6.5,\OriginY-4.5+0.7) circle (0.5cm) node[] at (\OriginX+6.5,\OriginY+2*\IncrY-5.7) {\Huge B};

\draw [black, line width=0.5mm] (\OriginX+8.0,\OriginY-5.0) circle (0.5cm) node[] at (\OriginX+8.0,\OriginY-5.0) {\Huge C};
\draw [black, line width=0.5mm] (\OriginX+8.0,\OriginY-4.5+1.2) circle (0.5cm) node[] at (\OriginX+8.0,\OriginY-3.3) {\Huge D};

\node (a) at (\OriginX+3.7, \OriginY-6.4) {\Huge (b) };


%\draw [thick, ->, line width=0.5mm] (\OriginX+5.3, \OriginY-1.0) -- (\OriginX+10.0, \OriginY-1.0);
%\node (a) at (\OriginX+7.7, \OriginY-1.8) {\Large (b) Latent Space};

%\draw [black,thick, line width=0.5mm] (\OriginX+6.6,\OriginY) circle (0.5cm) node[] at (\OriginX+6.6,\OriginY) {\Huge 646};
%\draw [red,thick, line width=0.5mm] (\OriginX+9.6,\OriginY+1.5) circle (0.5cm) node[] at (\OriginX+9.6,\OriginY+1.5) {\Huge 646};
%\draw [blue,thick, line width=0.5mm] (\OriginX+6.9,\OriginY+1.5) circle (0.5cm) node[] at (\OriginX+6.9,\OriginY+1.5) {\Huge 646};

%\node (g) at (\OriginX+5.6, \OriginY-0.3) {\Huge t=7};
%\node (h) at (\OriginX+6.6, \OriginY+2.3) {\Huge t=8 ??};
%\node (i) at (\OriginX+9.2, \OriginY+0.7) {\Huge t=8 ??};

\end{tikzpicture}
%\vspace{-0.2in}
\caption{ (a) shows the periodicity of the neighborhood of a Node, A (Alice) at time, t=1, t=2, and t=3. (b) shows temporal latent positions for Alice (A) and three other nodes, B (Bob), C (Cynthia), and D (David) in those three time-stamps. With our temporal smoothness assumption, at time t=2, Alice should still be close to Bob (close to it's previous position); with network homophily Alice should be near Cynthia and David.  }
\label{temporal_smoothing}
%\vspace{-0.2in}
\end{figure}

==> relwork_temp.tex <==
\begin{itemize}
\item DeepWalk
\begin{enumerate}
\item 
\end{enumerate}
\item node2vec 
\begin{enumerate}
\item 
\end{enumerate}
\item LINE 
\begin{enumerate}
\item 
\end{enumerate}
\item Grarep
\item Learning latent representations of nodes for classifying in heterogeneous social networks
\item Semi-supervised classification with graph convolutional networks
\item Asymmetric transitivity preserving graph embedding
\item Non-transitive hashing with latent similarity components
\item PTE: Predictive text embedding through large-scale heterogeneous text networks
\item CANE: Context-Aware Network Embedding for Relation Modeling
\item Max-margin DeepWalk: discriminative learning of network representation
\item TransNet: Translation-Based Network Representation Learning for Social Relation Extraction
\item Structural deep network embedding
\item Community Preserving Network Embedding
\item Network representation learning with rich text information
\item Fast Network Embedding Enhancement via High Order Proximity Approximation
\item Revisiting Semi-Supervised Learning with Graph Embeddings
\item Heterogeneous Network Embedding via Deep Architectures
\item Deep Neural Networks for Learning Graph Representations
\item metapath2vec: Scalable Representation Learning for Heterogeneous Networks (printed)
\item Learning from Labeled and Unlabeled Vertices in Networks
\item Unsupervised Feature Selection in Signed Social Networks
\item struc2vec: Learning Node Representations from Structural Identity (printed)
\item Inductive Representation Learning on Large Graphs (printed)
\item Predictive Network Representation Learning for Link Prediction
\item Weisfeiler-Lehman Neural Machine for Link Prediction
\item FacetNet: A Framework for Analyzing Communities and Their Evolutions in Dynamic Networks
\item Evolutionary Spectral Clustering by Incorporating Temporal Smoothness
\item Semi-Supervised Classification with Graph Convolutional Networks (GCN)
\item Jointly Learning Word Representations and Composition Functions
Using Predicate-Argument Structures
\item A Comparison of Vector-based Representations for Semantic Composition

\end{itemize}

==> tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\scriptsize
\begin{table*}[]
\centering
\caption{dblp2 results}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc                         & auc                         & auprc                       & ndcg                        \\
bcgd                                                & 0.7409                      & 0.7932                      & 0.8023                      & 0.8686                      \\
bcgd                                                & 0.0215                      & 0.0378                      & 0.0337                      & 0.0288                      \\
deepwalk\_homogeneous\_linear\_projection           & \textbf{0.7085}                      & \textbf{0.7422}                      & \textbf{0.7691}                      & \textbf{0.8496}                      \\
deepwalk\_homogeneous\_linear\_projection           & 0.0316                      & 0.0315                      & 0.0429                      & 0.0559                      \\
line\_homogeneous\_linear\_projection               & 0.6201                      & 0.6542                      & 0.6408                      & 0.6700                      \\
line\_homogeneous\_linear\_projection               & 0.0546                      & 0.0633                      & 0.0580                      & 0.0896                      \\
node2vec\_homogeneous\_linear\_projection           & 0.6553                      & 0.6952                      & 0.7012                      & 0.7486                      \\
node2vec\_homogeneous\_linear\_projection           & 0.0412                      & 0.0422                      & 0.0457                      & 0.0595                      \\
pca\_homogeneous\_linear\_projection                & 0.5757                      & 0.6206                      & 0.6728                      & 0.7722                      \\
pca\_homogeneous\_linear\_projection                & 0.0236                      & 0.0265                      & 0.0292                      & 0.0376                      \\
tsvd\_homogeneous\_linear\_projection               & 0.5578                      & 0.6391                      & 0.6806                      & 0.8035                      \\
tsvd\_homogeneous\_linear\_projection               & 0.0202                      & 0.0461                      & 0.0458                      & 0.0601                      \\
lle\_homogeneous\_linear\_projection                & 0.5755                      & 0.5736                      & 0.6171                      & 0.6782                      \\
lle\_homogeneous\_linear\_projection                & 0.0303                      & 0.0262                      & 0.0236                      & 0.0478                      \\
isomap\_homogeneous\_linear\_projection             & 0.5940                      & 0.6483                      & 0.6946                      & 0.7737                      \\
isomap\_homogeneous\_linear\_projection             & 0.0249                      & 0.0278                      & 0.0299                      & 0.0500                      \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.6986                      & 0.7276                      & 0.7462                      & 0.8174                      \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0233                      & 0.0287                      & 0.0354                      & 0.0404                      \\
line\_heterogeneous\_linear\_projection\_wct        & 0.6529                      & 0.6996                      & 0.7310                      & 0.8085                      \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0314                      & 0.0390                      & 0.0335                      & 0.0407                      \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.6986                      & 0.7340                      & 0.7432                      & 0.8085                      \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0369                      & 0.0301                      & 0.0329                      & 0.0483                      \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6252                      & 0.6473                      & 0.7011                      & 0.8123                      \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0164                      & 0.0294                      & 0.0276                      & 0.0300                      \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6431                      & 0.6642                      & 0.7136                      & 0.8251                      \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0174                      & 0.0385                      & 0.0303                      & 0.0392                      \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5848                      & 0.5631                      & 0.6437                      & 0.7204                      \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0142                      & 0.0220                      & 0.0233                      & 0.0447                      \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6154                      & 0.6468                      & 0.7001                      & 0.7784                      \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0209                      & 0.0330                      & 0.0243                      & 0.0377                      \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & \textbf{0.6991}                     & \textbf{0.7413}                      & \textbf{0.7798}                      & \textbf{0.8682}                      \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0313                      & 0.0257                      & 0.0264                      & 0.0274                      \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6426                      & 0.6842                      & 0.6827                      & 0.7277                      \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0406                      & 0.0495                      & 0.0509                      & 0.0643                      \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.7014                      & 0.7430                      & 0.7665                      & 0.8445                      \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0260                      & 0.0263                      & 0.0197                      & 0.0254                      \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5761                      & 0.6096                      & 0.6599                      & 0.7558                      \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0211                      & 0.0287                      & 0.0350                      & 0.0500                      \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5650                      & 0.6377                      & 0.6765                      & 0.7926                      \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0206                      & 0.0457                      & 0.0440                      & 0.0592                      \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5799                      & 0.5489                      & 0.6286                      & 0.6999                      \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0242                      & 0.0215                      & 0.0141                      & 0.0264                      \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6047                      & 0.6363                      & 0.6932                      & 0.7761                      \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0191                      & 0.0250                      & 0.0205                      & 0.0396                      \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.6803                      & 0.6983                      & 0.7158                      & 0.7848                      \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0339                      & 0.0301                      & 0.0275                      & 0.0309                      \\
line\_heterogeneous\_linear\_projection\_linear     & 0.6627                      & 0.6941                      & 0.7219                      & 0.8014                      \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0422                      & 0.0429                      & 0.0421                      & 0.0491                      \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.6938                      & 0.7229                      & 0.7376                      & 0.8116                      \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0187                      & 0.0172                      & 0.0289                      & 0.0419                      \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6255                      & 0.6188                      & 0.6843                      & 0.7892                      \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0136                      & 0.0260                      & 0.0205                      & 0.0186                      \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6514                      & 0.6902                      & 0.7290                      & 0.8418                      \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0258                      & 0.0319                      & 0.0277                      & 0.0350                      \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5750                      & 0.5455                      & 0.6276                      & 0.6946                      \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0168                      & 0.0241                      & 0.0179                      & 0.0292                      \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6201                      & 0.6650                      & 0.7151                      & 0.7947                      \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0208                      & 0.0332                      & 0.0232                      & 0.0326                      \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.6810                      & 0.6935                      & 0.7066                      & 0.7645                      \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0253                      & 0.0256                      & 0.0344                      & 0.0502                      \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6576                      & 0.6771                      & 0.6959                      & 0.7658                      \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0301                      & 0.0339                      & 0.0388                      & 0.0475                      \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.6848                      & 0.6975                      & 0.6971                      & 0.7640                      \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0276                      & 0.0305                      & 0.0354                      & 0.0420                      \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6217                      & 0.6152                      & 0.6733                      & 0.7822                      \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0279                      & 0.0205                      & 0.0269                      & 0.0381                      \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6495                      & 0.6518                      & 0.7039                      & 0.8189                      \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0267                      & 0.0368                      & 0.0297                      & 0.0416                      \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5745                      & 0.5470                      & 0.6269                      & 0.6966                      \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0172                      & 0.0210                      & 0.0118                      & 0.0186                      \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6216                      & 0.6007                      & 0.6658                      & 0.7657                      \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0236                      & 0.0350                      & 0.0396                      & 0.0472                      \\
deepwalk\_iterupdate                                & 0.6821                      & 0.7694                      & 0.7808                      & 0.8412                      \\
deepwalk\_iterupdate                                & 0.0366                      & 0.0364                      & 0.0357                      & 0.0435                      \\
line\_iterupdate                                    & 0.6582                      & 0.7452                      & 0.7605                      & 0.8166                      \\
line\_iterupdate                                    & 0.0434                      & 0.0487                      & 0.0443                      & 0.0416                      \\
node2vec\_iterupdate                                & 0.6511                      & 0.7376                      & 0.7669                      & 0.8377                      \\
node2vec\_iterupdate                                & 0.0420                      & 0.0493                      & 0.0385                      & 0.0357                      \\
pca\_iterupdate                                     & 0.6114                      & 0.8321                      & 0.8474                      & 0.9286                      \\
pca\_iterupdate                                     & 0.0252                      & 0.0132                      & 0.0112                      & 0.0245                      \\
tsvd\_iterupdate                                    & 0.6163                      & 0.8360                      & 0.8571                      & 0.9317                      \\
tsvd\_iterupdate                                    & 0.0215                      & 0.0234                      & 0.0197                      & 0.0241                      \\
lle\_iterupdate                                     & 0.5989                      & 0.8368                      & 0.8453                      & 0.8967                      \\
lle\_iterupdate                                     & 0.0269                      & 0.0363                      & 0.0326                      & 0.0366                      \\ 
{isomap\_iterupdate}             & {0.6125} &{0.8187} &{0.8346} & {0.9098} \\
isomap\_iterupdate                                  & 0.0236                      & 0.0234                      & 0.0184                      & 0.0274                     
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{dblp3 results (64)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.7782 & 0.8564 & 0.8599 & 0.9524 \\
bcgd                                                & 0.0176 & 0.0168 & 0.0202 & 0.0242 \\
deepwalk\_homogeneous\_linear\_projection           & 0.7569 & 0.8073 & 0.8087 & 0.9132 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0176 & 0.0180 & 0.0199 & 0.0316 \\
line\_homogeneous\_linear\_projection               & 0.6841 & 0.7557 & 0.7818 & 0.9671 \\
line\_homogeneous\_linear\_projection               & 0.0213 & 0.0233 & 0.0204 & 0.0166 \\
node2vec\_homogeneous\_linear\_projection           & 0.7039 & 0.7669 & 0.7706 & 0.8968 \\
node2vec\_homogeneous\_linear\_projection           & 0.0185 & 0.0194 & 0.0209 & 0.0330 \\
pca\_homogeneous\_linear\_projection                & 0.6033 & 0.7359 & 0.7735 & 0.9777 \\
pca\_homogeneous\_linear\_projection                & 0.0109 & 0.0131 & 0.0127 & 0.0139 \\
tsvd\_homogeneous\_linear\_projection               & 0.6220 & 0.7367 & 0.7724 & 0.9827 \\
tsvd\_homogeneous\_linear\_projection               & 0.0070 & 0.0188 & 0.0150 & 0.0169 \\
lle\_homogeneous\_linear\_projection                & 0.6257 & 0.6407 & 0.6990 & 0.9353 \\
lle\_homogeneous\_linear\_projection                & 0.0152 & 0.0195 & 0.0184 & 0.0332 \\
isomap\_homogeneous\_linear\_projection             & 0.6190 & 0.6874 & 0.7479 & 0.9762 \\
isomap\_homogeneous\_linear\_projection             & 0.0132 & 0.0166 & 0.0150 & 0.0114 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.7787 & 0.8344 & 0.8538 & 0.9683 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0107 & 0.0123 & 0.0148 & 0.0225 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.7690 & 0.8265 & 0.8607 & 0.9831 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0108 & 0.0127 & 0.0093 & 0.0217 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7899 & 0.8391 & 0.8566 & 0.9608 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0138 & 0.0120 & 0.0104 & 0.0129 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.7139 & 0.7734 & 0.8177 & 0.9864 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0136 & 0.0167 & 0.0140 & 0.0123 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6929 & 0.7630 & 0.8044 & 0.9912 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0158 & 0.0217 & 0.0176 & 0.0105 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.6474 & 0.6870 & 0.7500 & 0.9859 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0114 & 0.0164 & 0.0156 & 0.0150 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6635 & 0.7262 & 0.7769 & 0.9850 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0102 & 0.0234 & 0.0174 & 0.0130 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.7854 & 0.8341 & 0.8579 & 0.9794 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0146 & 0.0140 & 0.0118 & 0.0080 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.7511 & 0.8048 & 0.8360 & 0.9785 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0199 & 0.0222 & 0.0212 & 0.0183 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.7401 & 0.8004 & 0.8155 & 0.9507 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0142 & 0.0147 & 0.0216 & 0.0320 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.6065 & 0.7372 & 0.7776 & 0.9790 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0117 & 0.0143 & 0.0140 & 0.0152 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.6194 & 0.7356 & 0.7685 & 0.9724 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0076 & 0.0178 & 0.0153 & 0.0252 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.6478 & 0.6807 & 0.7452 & 0.9912 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0138 & 0.0221 & 0.0167 & 0.0073 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6139 & 0.6799 & 0.7445 & 0.9706 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0142 & 0.0255 & 0.0217 & 0.0149 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.7806 & 0.8371 & 0.8563 & 0.9751 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0141 & 0.0132 & 0.0139 & 0.0141 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.7765 & 0.8301 & 0.8680 & 0.9934 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0060 & 0.0115 & 0.0071 & 0.0041 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7900 & 0.8442 & 0.8636 & 0.9676 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0155 & 0.0137 & 0.0150 & 0.0167 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.7212 & 0.7781 & 0.8222 & 0.9884 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0114 & 0.0151 & 0.0137 & 0.0094 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.7049 & 0.7546 & 0.7987 & 0.9841 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0160 & 0.0170 & 0.0153 & 0.0134 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.6500 & 0.6884 & 0.7517 & 0.9911 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0121 & 0.0160 & 0.0152 & 0.0120 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6717 & 0.7156 & 0.7727 & 0.9837 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0117 & 0.0165 & 0.0144 & 0.0145 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.7767 & 0.8334 & 0.8513 & 0.9667 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0104 & 0.0125 & 0.0123 & 0.0110 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.7726 & 0.8263 & 0.8611 & 0.9852 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0109 & 0.0104 & 0.0087 & 0.0100 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7914 & 0.8474 & 0.8660 & 0.9713 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0112 & 0.0143 & 0.0115 & 0.0098 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.7262 & 0.7722 & 0.8188 & 0.9887 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0140 & 0.0148 & 0.0137 & 0.0061 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.7186 & 0.7497 & 0.7956 & 0.9786 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0126 & 0.0161 & 0.0174 & 0.0169 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.6511 & 0.6848 & 0.7490 & 0.9928 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0134 & 0.0200 & 0.0170 & 0.0117 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6670 & 0.6995 & 0.7591 & 0.9798 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0147 & 0.0136 & 0.0129 & 0.0120 \\
deepwalk\_iterupdate                                & 0.7606 & 0.8395 & 0.8502 & 0.9760 \\
deepwalk\_iterupdate                                & 0.0244 & 0.0259 & 0.0226 & 0.0121 \\
line\_iterupdate                                    & 0.7574 & 0.8367 & 0.8544 & 0.9811 \\
line\_iterupdate                                    & 0.0184 & 0.0203 & 0.0201 & 0.0199 \\
node2vec\_iterupdate                                & 0.7679 & 0.8463 & 0.8567 & 0.9777 \\
node2vec\_iterupdate                                & 0.0164 & 0.0178 & 0.0141 & 0.0141 \\
pca\_iterupdate                                     & 0.6690 & 0.8535 & 0.8570 & 0.9514 \\
pca\_iterupdate                                     & 0.0214 & 0.0114 & 0.0166 & 0.0283 \\
tsvd\_iterupdate                                    & 0.6677 & 0.8074 & 0.8245 & 0.9503 \\
tsvd\_iterupdate                                    & 0.0153 & 0.0445 & 0.0396 & 0.0291 \\
lle\_iterupdate                                     & 0.6370 & 0.8898 & 0.8926 & 0.9776 \\
lle\_iterupdate                                     & 0.0119 & 0.0138 & 0.0134 & 0.0162 \\
isomap\_iterupdate                                  & 0.6580 & 0.8154 & 0.8275 & 0.9605 \\
isomap\_iterupdate                                  & 0.0170 & 0.0307 & 0.0258 & 0.0206
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Facebook 2 Results (64)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.6941 & 0.7537 & 0.7190 & 0.7957 \\
bcgd                                                & 0.0229 & 0.0242 & 0.0239 & 0.0543 \\
deepwalk\_homogeneous\_linear\_projection           & 0.6618 & 0.7252 & 0.7144 & 0.8422 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0164 & 0.0207 & 0.0228 & 0.0369 \\
line\_homogeneous\_linear\_projection               & 0.6416 & 0.6854 & 0.6954 & 0.8596 \\
line\_homogeneous\_linear\_projection               & 0.0152 & 0.0179 & 0.0164 & 0.0297 \\
node2vec\_homogeneous\_linear\_projection           & 0.6586 & 0.7070 & 0.6931 & 0.8016 \\
node2vec\_homogeneous\_linear\_projection           & 0.0219 & 0.0248 & 0.0306 & 0.0563 \\
pca\_homogeneous\_linear\_projection                & 0.5923 & 0.6430 & 0.6669 & 0.8902 \\
pca\_homogeneous\_linear\_projection                & 0.0112 & 0.0192 & 0.0175 & 0.0265 \\
tsvd\_homogeneous\_linear\_projection               & 0.5993 & 0.6634 & 0.6716 & 0.8377 \\
tsvd\_homogeneous\_linear\_projection               & 0.0121 & 0.0199 & 0.0176 & 0.0249 \\
lle\_homogeneous\_linear\_projection                & 0.5644 & 0.5564 & 0.5766 & 0.6724 \\
lle\_homogeneous\_linear\_projection                & 0.0143 & 0.0203 & 0.0137 & 0.0313 \\
isomap\_homogeneous\_linear\_projection             & 0.5787 & 0.6083 & 0.6428 & 0.8587 \\
isomap\_homogeneous\_linear\_projection             & 0.0112 & 0.0150 & 0.0160 & 0.0311 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.6978 & 0.7580 & 0.7551 & 0.8947 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0116 & 0.0101 & 0.0128 & 0.0233 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.6866 & 0.7362 & 0.7598 & 0.9388 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0146 & 0.0162 & 0.0118 & 0.0171 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7078 & 0.7712 & 0.7671 & 0.8956 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0176 & 0.0189 & 0.0148 & 0.0188 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6404 & 0.6899 & 0.7215 & 0.9197 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0128 & 0.0173 & 0.0186 & 0.0257 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6401 & 0.6967 & 0.7268 & 0.9375 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0132 & 0.0090 & 0.0141 & 0.0391 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5613 & 0.5487 & 0.5969 & 0.7938 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0118 & 0.0148 & 0.0182 & 0.0556 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.5908 & 0.5975 & 0.6486 & 0.8793 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0118 & 0.0170 & 0.0156 & 0.0256 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.6789 & 0.7488 & 0.7471 & 0.8958 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0157 & 0.0160 & 0.0184 & 0.0328 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6569 & 0.6999 & 0.7112 & 0.8675 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0182 & 0.0212 & 0.0211 & 0.0358 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.6619 & 0.7176 & 0.7028 & 0.8157 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0121 & 0.0134 & 0.0229 & 0.0704 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5874 & 0.6385 & 0.6625 & 0.8839 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0088 & 0.0193 & 0.0153 & 0.0200 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5969 & 0.6483 & 0.6666 & 0.8438 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0133 & 0.0214 & 0.0196 & 0.0375 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5534 & 0.5481 & 0.5937 & 0.8066 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0154 & 0.0133 & 0.0149 & 0.0439 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.5806 & 0.5865 & 0.6317 & 0.8420 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0128 & 0.0137 & 0.0152 & 0.0295 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.6960 & 0.7562 & 0.7509 & 0.8930 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0150 & 0.0099 & 0.0095 & 0.0200 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.6825 & 0.7375 & 0.7583 & 0.9178 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0113 & 0.0155 & 0.0122 & 0.0187 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7137 & 0.7792 & 0.7788 & 0.9200 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0163 & 0.0174 & 0.0177 & 0.0164 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6437 & 0.6825 & 0.7163 & 0.9188 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0148 & 0.0180 & 0.0204 & 0.0278 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6380 & 0.6884 & 0.7217 & 0.9350 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0157 & 0.0200 & 0.0176 & 0.0314 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5584 & 0.5496 & 0.5926 & 0.7736 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0131 & 0.0131 & 0.0169 & 0.0770 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.5940 & 0.6039 & 0.6530 & 0.8832 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0139 & 0.0156 & 0.0170 & 0.0283 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.6888 & 0.7426 & 0.7375 & 0.8721 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0118 & 0.0123 & 0.0134 & 0.0208 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6857 & 0.7362 & 0.7591 & 0.9317 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0151 & 0.0168 & 0.0134 & 0.0254 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7111 & 0.7698 & 0.7667 & 0.9037 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0144 & 0.0128 & 0.0138 & 0.0162 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6433 & 0.6684 & 0.7071 & 0.9136 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0111 & 0.0106 & 0.0129 & 0.0170 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6473 & 0.6781 & 0.7177 & 0.9340 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0112 & 0.0177 & 0.0125 & 0.0239 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5609 & 0.5499 & 0.5937 & 0.7835 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0163 & 0.0091 & 0.0144 & 0.0615 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.5860 & 0.5867 & 0.6355 & 0.8524 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0102 & 0.0125 & 0.0129 & 0.0250 \\
deepwalk\_iterupdate                                & 0.7145 & 0.8199 & 0.8079 & 0.9439 \\
deepwalk\_iterupdate                                & 0.0227 & 0.0190 & 0.0197 & 0.0160 \\
line\_iterupdate                                    & 0.6869 & 0.7871 & 0.7882 & 0.9445 \\
line\_iterupdate                                    & 0.0240 & 0.0291 & 0.0263 & 0.0214 \\
node2vec\_iterupdate                                & 0.7210 & 0.7890 & 0.7286 & 0.7816 \\
node2vec\_iterupdate                                & 0.0114 & 0.0190 & 0.0297 & 0.0683 \\
pca\_iterupdate                                     & 0.6531 & 0.8202 & 0.8144 & 0.9519 \\
pca\_iterupdate                                     & 0.0140 & 0.0164 & 0.0159 & 0.0242 \\
tsvd\_iterupdate                                    & 0.6470 & 0.7785 & 0.7800 & 0.9581 \\
tsvd\_iterupdate                                    & 0.0159 & 0.0185 & 0.0188 & 0.0245 \\
lle\_iterupdate                                     & 0.6347 & 0.7625 & 0.7541 & 0.9335 \\
lle\_iterupdate                                     & 0.0754 & 0.1580 & 0.1583 & 0.0344 \\
isomap\_iterupdate                                  & 0.6569 & 0.8163 & 0.8153 & 0.9454 \\
isomap\_iterupdate                                  & 0.0164 & 0.0245 & 0.0183 & 0.0214
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{CollegeMSG (64)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.5958 & 0.6663 & 0.6691 & 0.7266 \\
bcgd                                                & 0.0126 & 0.0152 & 0.0209 & 0.0650 \\
deepwalk\_homogeneous\_linear\_projection           & 0.6364 & 0.5942 & 0.6500 & 0.7700 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0140 & 0.0199 & 0.0162 & 0.0356 \\
line\_homogeneous\_linear\_projection               & 0.6887 & 0.7460 & 0.7788 & 0.9571 \\
line\_homogeneous\_linear\_projection               & 0.0076 & 0.0164 & 0.0152 & 0.0171 \\
node2vec\_homogeneous\_linear\_projection           & 0.7100 & 0.7159 & 0.7113 & 0.7277 \\
node2vec\_homogeneous\_linear\_projection           & 0.0094 & 0.0119 & 0.0137 & 0.0483 \\
pca\_homogeneous\_linear\_projection                & 0.5870 & 0.5063 & 0.5885 & 0.9741 \\
pca\_homogeneous\_linear\_projection                & 0.0072 & 0.0072 & 0.0092 & 0.0240 \\
tsvd\_homogeneous\_linear\_projection               & 0.6698 & 0.7202 & 0.7382 & 0.9763 \\
tsvd\_homogeneous\_linear\_projection               & 0.0089 & 0.0101 & 0.0095 & 0.0149 \\
lle\_homogeneous\_linear\_projection                & 0.5949 & 0.4929 & 0.5869 & 0.8494 \\
lle\_homogeneous\_linear\_projection                & 0.0119 & 0.0196 & 0.0206 & 0.0534 \\
isomap\_homogeneous\_linear\_projection             & 0.6071 & 0.4992 & 0.6350 & 0.9517 \\
isomap\_homogeneous\_linear\_projection             & 0.0104 & 0.0167 & 0.0138 & 0.0224 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.6605 & 0.6531 & 0.6983 & 0.8324 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0144 & 0.0219 & 0.0197 & 0.0347 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.7091 & 0.7517 & 0.7913 & 0.9685 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0093 & 0.0137 & 0.0084 & 0.0182 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7142 & 0.7285 & 0.7491 & 0.8459 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0108 & 0.0133 & 0.0169 & 0.0461 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6208 & 0.5528 & 0.6269 & 0.9792 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0116 & 0.0205 & 0.0165 & 0.0180 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6801 & 0.7080 & 0.7300 & 0.9767 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0129 & 0.0276 & 0.0192 & 0.0144 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5944 & 0.4938 & 0.6034 & 0.8685 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0156 & 0.0248 & 0.0240 & 0.0542 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6061 & 0.5113 & 0.6402 & 0.9397 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0130 & 0.0307 & 0.0244 & 0.0235 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.6711 & 0.6727 & 0.7097 & 0.8374 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0126 & 0.0151 & 0.0212 & 0.0475 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6894 & 0.7459 & 0.7805 & 0.9527 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0127 & 0.0225 & 0.0192 & 0.0236 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.7060 & 0.7092 & 0.6961 & 0.6734 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0106 & 0.0138 & 0.0194 & 0.0481 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5872 & 0.5041 & 0.5859 & 0.9691 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0078 & 0.0101 & 0.0106 & 0.0247 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.6672 & 0.7186 & 0.7369 & 0.9770 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0085 & 0.0102 & 0.0094 & 0.0161 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.6033 & 0.5143 & 0.5692 & 0.8593 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0091 & 0.0130 & 0.0123 & 0.0605 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6160 & 0.5141 & 0.6473 & 0.9614 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0085 & 0.0108 & 0.0108 & 0.0130 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.6746 & 0.6781 & 0.7153 & 0.8407 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0079 & 0.0134 & 0.0077 & 0.0277 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.7026 & 0.7426 & 0.7859 & 0.9685 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0091 & 0.0198 & 0.0143 & 0.0112 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7144 & 0.7260 & 0.7519 & 0.8623 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0105 & 0.0156 & 0.0173 & 0.0498 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6173 & 0.5473 & 0.6229 & 0.9787 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0076 & 0.0168 & 0.0140 & 0.0200 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6886 & 0.7264 & 0.7408 & 0.9772 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0088 & 0.0158 & 0.0136 & 0.0168 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5928 & 0.5062 & 0.6126 & 0.8673 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0119 & 0.0188 & 0.0198 & 0.0650 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6089 & 0.5178 & 0.6454 & 0.9501 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0090 & 0.0219 & 0.0181 & 0.0185 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.6752 & 0.6626 & 0.7018 & 0.8153 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0117 & 0.0136 & 0.0183 & 0.0442 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6977 & 0.7259 & 0.7760 & 0.9641 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0085 & 0.0199 & 0.0156 & 0.0180 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7117 & 0.7198 & 0.7469 & 0.8568 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0086 & 0.0115 & 0.0147 & 0.0318 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6197 & 0.5385 & 0.6165 & 0.9719 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0093 & 0.0164 & 0.0153 & 0.0207 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6895 & 0.6952 & 0.7229 & 0.9817 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0141 & 0.0185 & 0.0157 & 0.0169 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5951 & 0.4987 & 0.6114 & 0.8567 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0107 & 0.0197 & 0.0183 & 0.0469 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6135 & 0.5199 & 0.6477 & 0.9575 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0089 & 0.0217 & 0.0170 & 0.0157 \\
deepwalk\_iterupdate                                & 0.6088 & 0.7071 & 0.6420 & 0.5286 \\
deepwalk\_iterupdate                                & 0.0507 & 0.0960 & 0.0624 & 0.0638 \\
line\_iterupdate                                    & 0.5527 & 0.5774 & 0.5900 & 0.7486 \\
line\_iterupdate                                    & 0.0099 & 0.0194 & 0.0123 & 0.0609 \\
node2vec\_iterupdate                                & 0.5840 & 0.6292 & 0.5962 & 0.5990 \\
node2vec\_iterupdate                                & 0.0091 & 0.0056 & 0.0080 & 0.0312 \\
pca\_iterupdate                                     & 0.5668 & 0.6291 & 0.6435 & 0.8381 \\
pca\_iterupdate                                     & 0.0066 & 0.0168 & 0.0202 & 0.0690 \\
tsvd\_iterupdate                                    & 0.6063 & 0.6398 & 0.6372 & 0.7188 \\
tsvd\_iterupdate                                    & 0.0595 & 0.1087 & 0.0536 & 0.1234 \\
lle\_iterupdate                                     & 0.5399 & 0.5506 & 0.5723 & 0.7226 \\
lle\_iterupdate                                     & 0.0640 & 0.0872 & 0.0555 & 0.0814 \\
isomap\_iterupdate                                  & 0.5451 & 0.6000 & 0.5863 & 0.6560 \\
isomap\_iterupdate                                  & 0.0092 & 0.0108 & 0.0120 & 0.0461
\end{tabular}
\end{table*}




\begin{table*}[]
\centering
\caption{Email EU (64)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.5623 & 0.6215 & 0.5946 & 0.6154 \\
bcgd                                                & 0.0098 & 0.0142 & 0.0226 & 0.1395 \\
deepwalk\_homogeneous\_linear\_projection           & 0.6318 & 0.7189 & 0.6762 & 0.7485 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0098 & 0.0182 & 0.0128 & 0.0505 \\
line\_homogeneous\_linear\_projection               & 0.7954 & 0.8789 & 0.8694 & 0.9705 \\
line\_homogeneous\_linear\_projection               & 0.0080 & 0.0098 & 0.0102 & 0.0168 \\
node2vec\_homogeneous\_linear\_projection           & 0.6796 & 0.7279 & 0.6477 & 0.6145 \\
node2vec\_homogeneous\_linear\_projection           & 0.0211 & 0.0170 & 0.0162 & 0.0474 \\
pca\_homogeneous\_linear\_projection                & 0.7029 & 0.7332 & 0.8008 & 0.9926 \\
pca\_homogeneous\_linear\_projection                & 0.0050 & 0.0134 & 0.0098 & 0.0094 \\
tsvd\_homogeneous\_linear\_projection               & 0.7445 & 0.8829 & 0.8750 & 0.9892 \\
tsvd\_homogeneous\_linear\_projection               & 0.0089 & 0.0093 & 0.0083 & 0.0116 \\
lle\_homogeneous\_linear\_projection                & 0.6559 & 0.6067 & 0.6733 & 0.8919 \\
lle\_homogeneous\_linear\_projection                & 0.0089 & 0.0168 & 0.0133 & 0.0278 \\
isomap\_homogeneous\_linear\_projection             & 0.6947 & 0.7600 & 0.8179 & 0.9948 \\
isomap\_homogeneous\_linear\_projection             & 0.0080 & 0.0080 & 0.0078 & 0.0090 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.7762 & 0.8499 & 0.8474 & 0.9453 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0101 & 0.0099 & 0.0104 & 0.0234 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.8593 & 0.9211 & 0.9283 & 0.9923 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0053 & 0.0082 & 0.0066 & 0.0083 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7866 & 0.8598 & 0.8365 & 0.9314 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0122 & 0.0114 & 0.0152 & 0.0163 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.7901 & 0.8186 & 0.8708 & 0.9959 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0103 & 0.0106 & 0.0092 & 0.0082 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.8235 & 0.9003 & 0.9099 & 0.9912 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0086 & 0.0067 & 0.0062 & 0.0090 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.6989 & 0.6971 & 0.7762 & 0.9789 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0123 & 0.0200 & 0.0145 & 0.0140 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.7493 & 0.7487 & 0.8234 & 0.9949 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0107 & 0.0128 & 0.0085 & 0.0093 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.6832 & 0.7791 & 0.7345 & 0.8173 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0096 & 0.0077 & 0.0125 & 0.0375 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.7865 & 0.8806 & 0.8693 & 0.9784 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0103 & 0.0083 & 0.0085 & 0.0146 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.6495 & 0.7024 & 0.6164 & 0.5309 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0177 & 0.0148 & 0.0139 & 0.0615 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.7048 & 0.7260 & 0.7945 & 0.9928 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0064 & 0.0121 & 0.0106 & 0.0075 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.7455 & 0.8805 & 0.8735 & 0.9884 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0084 & 0.0094 & 0.0088 & 0.0126 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.7218 & 0.7237 & 0.7913 & 0.9711 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0096 & 0.0146 & 0.0093 & 0.0231 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.7112 & 0.7575 & 0.8254 & 0.9904 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0074 & 0.0084 & 0.0070 & 0.0172 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.7817 & 0.8489 & 0.8457 & 0.9440 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0105 & 0.0086 & 0.0118 & 0.0254 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.8591 & 0.9175 & 0.9262 & 0.9933 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0056 & 0.0066 & 0.0042 & 0.0067 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7991 & 0.8680 & 0.8485 & 0.9477 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0133 & 0.0120 & 0.0109 & 0.0268 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.7954 & 0.8099 & 0.8632 & 0.9904 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0071 & 0.0064 & 0.0068 & 0.0165 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.8258 & 0.8854 & 0.9005 & 0.9932 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0096 & 0.0081 & 0.0095 & 0.0080 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.7128 & 0.7044 & 0.7809 & 0.9766 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0087 & 0.0142 & 0.0096 & 0.0171 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.7494 & 0.7589 & 0.8253 & 0.9891 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0090 & 0.0118 & 0.0097 & 0.0157 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.7791 & 0.8477 & 0.8435 & 0.9411 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0114 & 0.0099 & 0.0077 & 0.0300 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.8565 & 0.9177 & 0.9262 & 0.9909 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0060 & 0.0060 & 0.0054 & 0.0096 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7948 & 0.8617 & 0.8419 & 0.9296 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0123 & 0.0131 & 0.0120 & 0.0267 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.7988 & 0.8101 & 0.8637 & 0.9888 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0084 & 0.0087 & 0.0090 & 0.0169 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.8264 & 0.8829 & 0.8996 & 0.9943 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0072 & 0.0074 & 0.0083 & 0.0089 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.7274 & 0.7233 & 0.7934 & 0.9726 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0092 & 0.0153 & 0.0101 & 0.0261 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.7542 & 0.7660 & 0.8306 & 0.9900 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0083 & 0.0108 & 0.0092 & 0.0131 \\
deepwalk\_iterupdate                                & 0.7887 & 0.8669 & 0.8496 & 0.9121 \\
deepwalk\_iterupdate                                & 0.0101 & 0.0099 & 0.0139 & 0.0340 \\
line\_iterupdate                                    & 0.8204 & 0.9049 & 0.9009 & 0.9725 \\
line\_iterupdate                                    & 0.0056 & 0.0058 & 0.0091 & 0.0286 \\
node2vec\_iterupdate                                & 0.6162 & 0.5635 & 0.4906 & 0.0469 \\
node2vec\_iterupdate                                & 0.0055 & 0.0105 & 0.0075 & 0.0203 \\
pca\_iterupdate                                     & 0.8116 & 0.9071 & 0.8976 & 0.9726 \\
pca\_iterupdate                                     & 0.0112 & 0.0158 & 0.0205 & 0.0305 \\
tsvd\_iterupdate                                    & 0.8176 & 0.9021 & 0.8974 & 0.9763 \\
tsvd\_iterupdate                                    & 0.0132 & 0.0141 & 0.0189 & 0.0246 \\
lle\_iterupdate                                     & 0.7112 & 0.9157 & 0.9047 & 0.9780 \\
lle\_iterupdate                                     & 0.0114 & 0.0170 & 0.0209 & 0.0201 \\
isomap\_iterupdate                                  & 0.7559 & 0.8851 & 0.8807 & 0.9713 \\
isomap\_iterupdate                                  & 0.0348 & 0.0186 & 0.0253 & 0.0340
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Enron Results (64)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.7646 & 0.8494 & 0.8285 & 0.8223 \\
bcgd                                                & 0.0270 & 0.0278 & 0.0288 & 0.0340 \\
deepwalk\_homogeneous\_linear\_projection           & 0.8247 & 0.8782 & 0.8776 & 0.8936 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0231 & 0.0208 & 0.0172 & 0.0199 \\
line\_homogeneous\_linear\_projection               & 0.7146 & 0.7732 & 0.7475 & 0.7504 \\
line\_homogeneous\_linear\_projection               & 0.0352 & 0.0352 & 0.0429 & 0.0491 \\
node2vec\_homogeneous\_linear\_projection           & 0.8130 & 0.8734 & 0.8730 & 0.8852 \\
node2vec\_homogeneous\_linear\_projection           & 0.0198 & 0.0193 & 0.0225 & 0.0206 \\
pca\_homogeneous\_linear\_projection                & 0.7159 & 0.7689 & 0.8197 & 0.8756 \\
pca\_homogeneous\_linear\_projection                & 0.0281 & 0.0197 & 0.0188 & 0.0203 \\
tsvd\_homogeneous\_linear\_projection               & 0.7104 & 0.7283 & 0.7626 & 0.8206 \\
tsvd\_homogeneous\_linear\_projection               & 0.0260 & 0.0309 & 0.0344 & 0.0480 \\
lle\_homogeneous\_linear\_projection                & 0.6128 & 0.6158 & 0.6626 & 0.6882 \\
lle\_homogeneous\_linear\_projection                & 0.0354 & 0.0354 & 0.0342 & 0.0400 \\
isomap\_homogeneous\_linear\_projection             & 0.7122 & 0.6957 & 0.7611 & 0.8231 \\
isomap\_homogeneous\_linear\_projection             & 0.0335 & 0.0572 & 0.0467 & 0.0415 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.8456 & 0.9004 & 0.8873 & 0.9049 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0214 & 0.0169 & 0.0239 & 0.0269 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.7799 & 0.8181 & 0.8221 & 0.8409 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0366 & 0.0354 & 0.0423 & 0.0436 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.8586 & 0.9051 & 0.9019 & 0.9207 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0204 & 0.0223 & 0.0224 & 0.0250 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.7565 & 0.7834 & 0.8306 & 0.8779 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0311 & 0.0405 & 0.0300 & 0.0353 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6992 & 0.6831 & 0.7457 & 0.8107 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0282 & 0.0251 & 0.0303 & 0.0281 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.6984 & 0.7126 & 0.7706 & 0.8118 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0405 & 0.0353 & 0.0292 & 0.0371 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6768 & 0.6240 & 0.6897 & 0.7521 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0268 & 0.0389 & 0.0456 & 0.0510 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.8237 & 0.8818 & 0.8775 & 0.8968 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0277 & 0.0238 & 0.0264 & 0.0265 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.7518 & 0.8276 & 0.8166 & 0.8222 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0300 & 0.0237 & 0.0304 & 0.0278 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.8469 & 0.8950 & 0.8863 & 0.9027 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0210 & 0.0213 & 0.0271 & 0.0268 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.7188 & 0.7595 & 0.8142 & 0.8657 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0250 & 0.0225 & 0.0215 & 0.0278 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.7185 & 0.7219 & 0.7593 & 0.8175 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0272 & 0.0415 & 0.0560 & 0.0574 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.6969 & 0.7011 & 0.7587 & 0.7996 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0320 & 0.0598 & 0.0454 & 0.0391 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.7029 & 0.6596 & 0.7439 & 0.8027 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0278 & 0.0307 & 0.0330 & 0.0308 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.8242 & 0.8636 & 0.8570 & 0.8807 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0227 & 0.0204 & 0.0209 & 0.0164 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.7721 & 0.8043 & 0.8057 & 0.8237 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0241 & 0.0251 & 0.0349 & 0.0368 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.8521 & 0.8961 & 0.8804 & 0.8965 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0206 & 0.0175 & 0.0182 & 0.0193 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.7633 & 0.8037 & 0.8378 & 0.8868 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0263 & 0.0357 & 0.0294 & 0.0347 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.7174 & 0.6808 & 0.7229 & 0.7972 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0218 & 0.0193 & 0.0281 & 0.0336 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.6906 & 0.7074 & 0.7597 & 0.7945 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0497 & 0.0482 & 0.0411 & 0.0509 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6737 & 0.6107 & 0.6771 & 0.7376 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0269 & 0.0365 & 0.0509 & 0.0537 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.7977 & 0.8224 & 0.8063 & 0.8362 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0254 & 0.0296 & 0.0312 & 0.0251 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.7393 & 0.7250 & 0.7408 & 0.7850 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0281 & 0.0331 & 0.0296 & 0.0260 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.8227 & 0.8581 & 0.8560 & 0.8894 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0238 & 0.0310 & 0.0327 & 0.0223 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.7594 & 0.7697 & 0.8136 & 0.8672 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0350 & 0.0490 & 0.0413 & 0.0407 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.7094 & 0.6664 & 0.7031 & 0.7753 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0349 & 0.0398 & 0.0397 & 0.0424 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.6984 & 0.7147 & 0.7591 & 0.8036 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0391 & 0.0522 & 0.0379 & 0.0450 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6659 & 0.6005 & 0.6536 & 0.7211 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0162 & 0.0153 & 0.0291 & 0.0295 \\
deepwalk\_iterupdate                                & 0.8133 & 0.8955 & 0.8814 & 0.8764 \\
deepwalk\_iterupdate                                & 0.0270 & 0.0100 & 0.0147 & 0.0125 \\
line\_iterupdate                                    & 0.7188 & 0.8503 & 0.8656 & 0.8706 \\
line\_iterupdate                                    & 0.0260 & 0.0185 & 0.0182 & 0.0331 \\
node2vec\_iterupdate                                & 0.7260 & 0.8241 & 0.8173 & 0.8100 \\
node2vec\_iterupdate                                & 0.0165 & 0.0333 & 0.0377 & 0.0472 \\
pca\_iterupdate                                     & 0.7531 & 0.9050 & 0.8984 & 0.8994 \\
pca\_iterupdate                                     & 0.0189 & 0.0168 & 0.0197 & 0.0243 \\
tsvd\_iterupdate                                    & 0.8102 & 0.9124 & 0.9062 & 0.9163 \\
tsvd\_iterupdate                                    & 0.0195 & 0.0141 & 0.0230 & 0.0204 \\
lle\_iterupdate                                     & 0.7406 & 0.9282 & 0.9227 & 0.9311 \\
lle\_iterupdate                                     & 0.0386 & 0.0079 & 0.0137 & 0.0186 \\
isomap\_iterupdate                                  & 0.8234 & 0.9104 & 0.9037 & 0.9167 \\
isomap\_iterupdate                                  & 0.0262 & 0.0226 & 0.0253 & 0.0243
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{dblp2 (32)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.7393 & 0.7911 & 0.7936 & 0.8554 \\
bcgd                                                & 0.0314 & 0.0356 & 0.0301 & 0.0312 \\
deepwalk\_homogeneous\_linear\_projection           & 0.6656 & 0.7253 & 0.7363 & 0.8009 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0315 & 0.0208 & 0.0371 & 0.0519 \\
line\_homogeneous\_linear\_projection               & 0.6408 & 0.6803 & 0.6742 & 0.7234 \\
line\_homogeneous\_linear\_projection               & 0.0497 & 0.0518 & 0.0468 & 0.0533 \\
node2vec\_homogeneous\_linear\_projection           & 0.6214 & 0.6555 & 0.6406 & 0.6764 \\
node2vec\_homogeneous\_linear\_projection           & 0.0326 & 0.0442 & 0.0382 & 0.0424 \\
pca\_homogeneous\_linear\_projection                & 0.5920 & 0.6192 & 0.6879 & 0.7527 \\
pca\_homogeneous\_linear\_projection                & 0.0246 & 0.0324 & 0.0374 & 0.0508 \\
tsvd\_homogeneous\_linear\_projection               & 0.5770 & 0.6705 & 0.7161 & 0.8072 \\
tsvd\_homogeneous\_linear\_projection               & 0.0228 & 0.0313 & 0.0409 & 0.0431 \\
lle\_homogeneous\_linear\_projection                & 0.5736 & 0.6327 & 0.6664 & 0.7226 \\
lle\_homogeneous\_linear\_projection                & 0.0186 & 0.0313 & 0.0320 & 0.0396 \\
isomap\_homogeneous\_linear\_projection             & 0.5884 & 0.6541 & 0.6910 & 0.7670 \\
isomap\_homogeneous\_linear\_projection             & 0.0184 & 0.0319 & 0.0306 & 0.0447 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.7082 & 0.7537 & 0.7835 & 0.8659 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0270 & 0.0247 & 0.0268 & 0.0311 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.6598 & 0.7042 & 0.7151 & 0.7843 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0335 & 0.0363 & 0.0402 & 0.0505 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7076 & 0.7564 & 0.7715 & 0.8473 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0255 & 0.0308 & 0.0308 & 0.0306 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6234 & 0.6601 & 0.7215 & 0.8121 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0202 & 0.0305 & 0.0318 & 0.0409 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6207 & 0.6569 & 0.7249 & 0.8175 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0241 & 0.0265 & 0.0251 & 0.0327 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5766 & 0.5894 & 0.6408 & 0.6782 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0143 & 0.0327 & 0.0277 & 0.0372 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6031 & 0.6485 & 0.6948 & 0.7686 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0175 & 0.0423 & 0.0463 & 0.0605 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.7167 & 0.7669 & 0.8048 & 0.8950 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0155 & 0.0199 & 0.0194 & 0.0199 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6467 & 0.6862 & 0.6811 & 0.7311 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0416 & 0.0490 & 0.0457 & 0.0553 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.6225 & 0.6573 & 0.6443 & 0.6840 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0467 & 0.0472 & 0.0464 & 0.0581 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5848 & 0.6173 & 0.6752 & 0.7514 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0248 & 0.0330 & 0.0399 & 0.0531 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5716 & 0.6608 & 0.7109 & 0.8034 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0191 & 0.0291 & 0.0343 & 0.0450 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5527 & 0.5705 & 0.6197 & 0.6663 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0129 & 0.0552 & 0.0432 & 0.0528 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6038 & 0.6596 & 0.7065 & 0.7834 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0198 & 0.0197 & 0.0247 & 0.0382 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.7065 & 0.7534 & 0.7768 & 0.8522 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0258 & 0.0245 & 0.0222 & 0.0224 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.6589 & 0.7016 & 0.7131 & 0.7819 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0354 & 0.0385 & 0.0448 & 0.0497 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7056 & 0.7451 & 0.7629 & 0.8391 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0351 & 0.0347 & 0.0395 & 0.0407 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6245 & 0.6306 & 0.7049 & 0.7895 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0227 & 0.0269 & 0.0271 & 0.0356 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6386 & 0.6597 & 0.7275 & 0.8264 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0249 & 0.0391 & 0.0421 & 0.0567 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5793 & 0.6054 & 0.6599 & 0.7200 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0142 & 0.0377 & 0.0372 & 0.0535 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6087 & 0.6596 & 0.6979 & 0.7764 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0208 & 0.0255 & 0.0284 & 0.0480 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.7112 & 0.7423 & 0.7645 & 0.8475 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0285 & 0.0212 & 0.0237 & 0.0249 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6603 & 0.6924 & 0.7048 & 0.7713 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0364 & 0.0457 & 0.0486 & 0.0585 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7149 & 0.7538 & 0.7738 & 0.8476 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0321 & 0.0351 & 0.0355 & 0.0373 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6274 & 0.6362 & 0.7060 & 0.7944 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0253 & 0.0235 & 0.0260 & 0.0422 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6522 & 0.6760 & 0.7375 & 0.8328 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0306 & 0.0404 & 0.0427 & 0.0568 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5723 & 0.5854 & 0.6391 & 0.6921 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0124 & 0.0381 & 0.0339 & 0.0542 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6159 & 0.6439 & 0.6853 & 0.7685 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0292 & 0.0236 & 0.0386 & 0.0541 \\
deepwalk\_iterupdate                                & 0.6732 & 0.7668 & 0.7803 & 0.8482 \\
deepwalk\_iterupdate                                & 0.0346 & 0.0347 & 0.0251 & 0.0281 \\
line\_iterupdate                                    & 0.6264 & 0.7116 & 0.7322 & 0.7971 \\
line\_iterupdate                                    & 0.0404 & 0.0476 & 0.0466 & 0.0563 \\
node2vec\_iterupdate                                & 0.6565 & 0.7491 & 0.7635 & 0.8325 \\
node2vec\_iterupdate                                & 0.0378 & 0.0451 & 0.0359 & 0.0396 \\
pca\_iterupdate                                     & 0.5978 & 0.8230 & 0.8354 & 0.9116 \\
pca\_iterupdate                                     & 0.0233 & 0.0168 & 0.0183 & 0.0283 \\
tsvd\_iterupdate                                    & 0.6022 & 0.7887 & 0.8157 & 0.8970 \\
tsvd\_iterupdate                                    & 0.0183 & 0.0343 & 0.0319 & 0.0326 \\
lle\_iterupdate                                     & 0.6011 & 0.8121 & 0.8197 & 0.8779 \\
lle\_iterupdate                                     & 0.0297 & 0.0395 & 0.0378 & 0.0393 \\
isomap\_iterupdate                                  & 0.6092 & 0.8034 & 0.8249 & 0.9065 \\
isomap\_iterupdate                                  & 0.0205 & 0.0249 & 0.0273 & 0.0417
\end{tabular}
\end{table*}



\begin{table*}[]
\centering
\caption{dblp2 (128) }
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.7424 & 0.7965 & 0.8051 & 0.8728 \\
bcgd                                                & 0.0288 & 0.0338 & 0.0315 & 0.0310 \\
deepwalk\_homogeneous\_linear\_projection           & 0.7245 & 0.7732 & 0.8129 & 0.9042 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0237 & 0.0284 & 0.0256 & 0.0342 \\
line\_homogeneous\_linear\_projection               & 0.6402 & 0.6677 & 0.6476 & 0.6768 \\
line\_homogeneous\_linear\_projection               & 0.0342 & 0.0447 & 0.0484 & 0.0595 \\
node2vec\_homogeneous\_linear\_projection           & 0.6641 & 0.7301 & 0.7501 & 0.8263 \\
node2vec\_homogeneous\_linear\_projection           & 0.0416 & 0.0372 & 0.0337 & 0.0382 \\
pca\_homogeneous\_linear\_projection                & 0.5893 & 0.6128 & 0.6786 & 0.7603 \\
pca\_homogeneous\_linear\_projection                & 0.0232 & 0.0183 & 0.0272 & 0.0385 \\
tsvd\_homogeneous\_linear\_projection               & 0.5775 & 0.6526 & 0.7024 & 0.7959 \\
tsvd\_homogeneous\_linear\_projection               & 0.0177 & 0.0278 & 0.0333 & 0.0449 \\
lle\_homogeneous\_linear\_projection                & 0.5453 & 0.5616 & 0.6092 & 0.6678 \\
lle\_homogeneous\_linear\_projection                & 0.0409 & 0.0470 & 0.0442 & 0.0680 \\
isomap\_homogeneous\_linear\_projection             & 0.5868 & 0.6413 & 0.6731 & 0.7320 \\
isomap\_homogeneous\_linear\_projection             & 0.0253 & 0.0297 & 0.0345 & 0.0575 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.6882 & 0.7115 & 0.7148 & 0.7821 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0264 & 0.0259 & 0.0352 & 0.0430 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.6638 & 0.6965 & 0.7163 & 0.7899 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0234 & 0.0215 & 0.0282 & 0.0393 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7069 & 0.7241 & 0.7203 & 0.7842 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0247 & 0.0241 & 0.0230 & 0.0315 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6250 & 0.6396 & 0.7048 & 0.7934 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0171 & 0.0207 & 0.0287 & 0.0351 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6422 & 0.6625 & 0.7225 & 0.8189 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0295 & 0.0345 & 0.0362 & 0.0466 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5701 & 0.5639 & 0.6251 & 0.6924 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0130 & 0.0378 & 0.0311 & 0.0436 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6196 & 0.6175 & 0.6773 & 0.7701 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0332 & 0.0269 & 0.0325 & 0.0429 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.6995 & 0.7357 & 0.7459 & 0.8210 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0199 & 0.0265 & 0.0314 & 0.0370 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6641 & 0.7167 & 0.7472 & 0.8253 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0360 & 0.0335 & 0.0291 & 0.0392 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.7101 & 0.7424 & 0.7410 & 0.8074 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0238 & 0.0191 & 0.0267 & 0.0318 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5909 & 0.6209 & 0.6841 & 0.7708 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0167 & 0.0270 & 0.0346 & 0.0477 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5784 & 0.6491 & 0.6983 & 0.7833 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0175 & 0.0272 & 0.0298 & 0.0363 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5668 & 0.5710 & 0.6302 & 0.7039 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0425 & 0.0476 & 0.0408 & 0.0571 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6112 & 0.6421 & 0.6911 & 0.7772 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0229 & 0.0264 & 0.0340 & 0.0501 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.6757 & 0.6851 & 0.6912 & 0.7407 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0278 & 0.0256 & 0.0309 & 0.0349 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.6549 & 0.6747 & 0.7018 & 0.7817 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0279 & 0.0227 & 0.0270 & 0.0368 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.6844 & 0.6863 & 0.6759 & 0.7268 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0217 & 0.0103 & 0.0209 & 0.0468 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6368 & 0.6315 & 0.7079 & 0.8071 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0241 & 0.0382 & 0.0352 & 0.0399 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6516 & 0.6786 & 0.7343 & 0.8308 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0327 & 0.0218 & 0.0334 & 0.0452 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5543 & 0.5661 & 0.6279 & 0.6954 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0404 & 0.0574 & 0.0445 & 0.0593 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6196 & 0.6187 & 0.6789 & 0.7698 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0320 & 0.0333 & 0.0388 & 0.0538 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.6487 & 0.6626 & 0.6941 & 0.7099 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0275 & 0.0185 & 0.0215 & 0.0452 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6429 & 0.6341 & 0.6652 & 0.7434 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0238 & 0.0224 & 0.0311 & 0.0503 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.6547 & 0.6691 & 0.6808 & 0.7082 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0149 & 0.0190 & 0.0283 & 0.0503 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6263 & 0.6037 & 0.6858 & 0.7834 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0368 & 0.0428 & 0.0406 & 0.0513 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6500 & 0.6528 & 0.7200 & 0.8194 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0184 & 0.0285 & 0.0252 & 0.0281 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5543 & 0.5652 & 0.6250 & 0.6854 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0561 & 0.0586 & 0.0482 & 0.0588 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6116 & 0.5985 & 0.6609 & 0.7499 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0298 & 0.0270 & 0.0414 & 0.0563 \\
deepwalk\_iterupdate                                & 0.6583 & 0.7354 & 0.7605 & 0.8302 \\
deepwalk\_iterupdate                                & 0.0373 & 0.0353 & 0.0387 & 0.0514 \\
line\_iterupdate                                    & 0.6634 & 0.7470 & 0.7782 & 0.8463 \\
line\_iterupdate                                    & 0.0452 & 0.0559 & 0.0466 & 0.0516 \\
node2vec\_iterupdate                                & 0.6440 & 0.7123 & 0.7510 & 0.8330 \\
node2vec\_iterupdate                                & 0.0542 & 0.0624 & 0.0463 & 0.0460 \\
pca\_iterupdate                                     & 0.6109 & 0.8297 & 0.8462 & 0.9234 \\
pca\_iterupdate                                     & 0.0279 & 0.0240 & 0.0187 & 0.0111 \\
tsvd\_iterupdate                                    & 0.6087 & 0.8312 & 0.8528 & 0.9225 \\
tsvd\_iterupdate                                    & 0.0217 & 0.0328 & 0.0252 & 0.0249 \\
lle\_iterupdate                                     & 0.6141 & 0.8542 & 0.8679 & 0.9432 \\
lle\_iterupdate                                     & 0.0356 & 0.0247 & 0.0221 & 0.0266 \\
isomap\_iterupdate                                  & 0.6168 & 0.8311 & 0.8466 & 0.9279 \\
isomap\_iterupdate                                  & 0.0275 & 0.0180 & 0.0142 & 0.0196
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{dblp3 (32)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.7574 & 0.8473 & 0.8529 & 0.9566 \\
bcgd                                                & 0.0169 & 0.0170 & 0.0218 & 0.0252 \\
deepwalk\_homogeneous\_linear\_projection           & 0.7195 & 0.7863 & 0.7668 & 0.8439 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0145 & 0.0170 & 0.0169 & 0.0218 \\
line\_homogeneous\_linear\_projection               & 0.7047 & 0.7622 & 0.7651 & 0.8983 \\
line\_homogeneous\_linear\_projection               & 0.0127 & 0.0132 & 0.0145 & 0.0196 \\
node2vec\_homogeneous\_linear\_projection           & 0.7350 & 0.7937 & 0.7985 & 0.9220 \\
node2vec\_homogeneous\_linear\_projection           & 0.0196 & 0.0214 & 0.0263 & 0.0320 \\
pca\_homogeneous\_linear\_projection                & 0.6066 & 0.7623 & 0.8034 & 0.9837 \\
pca\_homogeneous\_linear\_projection                & 0.0089 & 0.0152 & 0.0142 & 0.0114 \\
tsvd\_homogeneous\_linear\_projection               & 0.6180 & 0.7430 & 0.7841 & 0.9785 \\
tsvd\_homogeneous\_linear\_projection               & 0.0051 & 0.0136 & 0.0114 & 0.0153 \\
lle\_homogeneous\_linear\_projection                & 0.5993 & 0.6172 & 0.6773 & 0.9380 \\
lle\_homogeneous\_linear\_projection                & 0.0085 & 0.0166 & 0.0167 & 0.0329 \\
isomap\_homogeneous\_linear\_projection             & 0.6193 & 0.7277 & 0.7692 & 0.9703 \\
isomap\_homogeneous\_linear\_projection             & 0.0099 & 0.0101 & 0.0127 & 0.0166 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.7599 & 0.8173 & 0.8263 & 0.9477 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0095 & 0.0107 & 0.0123 & 0.0177 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.7366 & 0.7923 & 0.8218 & 0.9702 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0107 & 0.0143 & 0.0111 & 0.0195 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7717 & 0.8239 & 0.8365 & 0.9437 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0079 & 0.0106 & 0.0104 & 0.0153 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6973 & 0.7802 & 0.8229 & 0.9901 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0162 & 0.0150 & 0.0134 & 0.0092 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6853 & 0.7719 & 0.8167 & 0.9884 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0156 & 0.0176 & 0.0143 & 0.0117 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.6108 & 0.6640 & 0.7149 & 0.9646 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0082 & 0.0145 & 0.0181 & 0.0344 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6614 & 0.7304 & 0.7781 & 0.9898 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0104 & 0.0237 & 0.0171 & 0.0122 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.7438 & 0.8097 & 0.8107 & 0.9259 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0161 & 0.0144 & 0.0205 & 0.0370 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6734 & 0.7448 & 0.7434 & 0.8924 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0114 & 0.0159 & 0.0167 & 0.0318 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.6647 & 0.7240 & 0.7078 & 0.8189 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0227 & 0.0241 & 0.0259 & 0.0494 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.6016 & 0.7525 & 0.7924 & 0.9804 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0087 & 0.0143 & 0.0129 & 0.0136 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.6172 & 0.7423 & 0.7801 & 0.9700 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0084 & 0.0158 & 0.0137 & 0.0220 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.6148 & 0.6420 & 0.7119 & 0.9902 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0076 & 0.0111 & 0.0089 & 0.0109 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6136 & 0.7089 & 0.7615 & 0.9789 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0126 & 0.0171 & 0.0174 & 0.0146 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.7591 & 0.8178 & 0.8255 & 0.9455 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0122 & 0.0120 & 0.0147 & 0.0162 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.7457 & 0.8014 & 0.8330 & 0.9826 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0126 & 0.0160 & 0.0159 & 0.0144 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7734 & 0.8262 & 0.8424 & 0.9639 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0144 & 0.0120 & 0.0123 & 0.0128 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.7057 & 0.7747 & 0.8188 & 0.9850 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0132 & 0.0179 & 0.0158 & 0.0127 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6921 & 0.7671 & 0.8123 & 0.9847 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0139 & 0.0160 & 0.0132 & 0.0117 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.6109 & 0.6643 & 0.7208 & 0.9939 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0081 & 0.0144 & 0.0127 & 0.0103 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6636 & 0.7212 & 0.7747 & 0.9836 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0084 & 0.0190 & 0.0169 & 0.0158 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.7566 & 0.8135 & 0.8211 & 0.9443 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0132 & 0.0120 & 0.0099 & 0.0198 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.7467 & 0.8007 & 0.8302 & 0.9738 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0156 & 0.0178 & 0.0190 & 0.0209 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7735 & 0.8283 & 0.8431 & 0.9589 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0141 & 0.0173 & 0.0190 & 0.0153 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.7147 & 0.7814 & 0.8235 & 0.9874 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0116 & 0.0103 & 0.0102 & 0.0085 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.7006 & 0.7630 & 0.8105 & 0.9839 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0104 & 0.0195 & 0.0159 & 0.0137 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.6089 & 0.6727 & 0.7282 & 0.9943 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0080 & 0.0118 & 0.0104 & 0.0069 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6650 & 0.7189 & 0.7708 & 0.9841 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0123 & 0.0159 & 0.0159 & 0.0145 \\
deepwalk\_iterupdate                                & 0.7675 & 0.8521 & 0.8559 & 0.9703 \\
deepwalk\_iterupdate                                & 0.0235 & 0.0224 & 0.0194 & 0.0119 \\
line\_iterupdate                                    & 0.7201 & 0.8058 & 0.8204 & 0.9759 \\
line\_iterupdate                                    & 0.0248 & 0.0268 & 0.0202 & 0.0162 \\
node2vec\_iterupdate                                & 0.7648 & 0.8390 & 0.8437 & 0.9674 \\
node2vec\_iterupdate                                & 0.0137 & 0.0152 & 0.0147 & 0.0106 \\
pca\_iterupdate                                     & 0.6467 & 0.8366 & 0.8387 & 0.9506 \\
pca\_iterupdate                                     & 0.0137 & 0.0200 & 0.0184 & 0.0273 \\
tsvd\_iterupdate                                    & 0.6533 & 0.7820 & 0.8011 & 0.9503 \\
tsvd\_iterupdate                                    & 0.0124 & 0.0423 & 0.0359 & 0.0291 \\
lle\_iterupdate                                     & 0.6161 & 0.8666 & 0.8616 & 0.9583 \\
lle\_iterupdate                                     & 0.0148 & 0.0166 & 0.0128 & 0.0154 \\
isomap\_iterupdate                                  & 0.6427 & 0.8014 & 0.8129 & 0.9603 \\
isomap\_iterupdate                                  & 0.0143 & 0.0356 & 0.0299 & 0.0208
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{dblp3 (128)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.7882 & 0.8607 & 0.8623 & 0.9434 \\
bcgd                                                & 0.0150 & 0.0138 & 0.0171 & 0.0326 \\
deepwalk\_homogeneous\_linear\_projection           & 0.7953 & 0.8469 & 0.8700 & 0.9768 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0110 & 0.0115 & 0.0118 & 0.0174 \\
line\_homogeneous\_linear\_projection               & 0.7444 & 0.8020 & 0.8371 & 0.9857 \\
line\_homogeneous\_linear\_projection               & 0.0170 & 0.0186 & 0.0185 & 0.0093 \\
node2vec\_homogeneous\_linear\_projection           & 0.7800 & 0.8331 & 0.8649 & 0.9878 \\
node2vec\_homogeneous\_linear\_projection           & 0.0153 & 0.0160 & 0.0110 & 0.0095 \\
pca\_homogeneous\_linear\_projection                & 0.6057 & 0.7228 & 0.7631 & 0.9775 \\
pca\_homogeneous\_linear\_projection                & 0.0111 & 0.0172 & 0.0183 & 0.0149 \\
tsvd\_homogeneous\_linear\_projection               & 0.6170 & 0.7154 & 0.7684 & 0.9752 \\
tsvd\_homogeneous\_linear\_projection               & 0.0062 & 0.0176 & 0.0147 & 0.0173 \\
lle\_homogeneous\_linear\_projection                & 0.6392 & 0.6414 & 0.7178 & 0.9921 \\
lle\_homogeneous\_linear\_projection                & 0.0147 & 0.0186 & 0.0148 & 0.0077 \\
isomap\_homogeneous\_linear\_projection             & 0.6165 & 0.7099 & 0.7521 & 0.9516 \\
isomap\_homogeneous\_linear\_projection             & 0.0096 & 0.0125 & 0.0122 & 0.0188 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.7510 & 0.7995 & 0.7998 & 0.9052 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0110 & 0.0106 & 0.0145 & 0.0299 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.7750 & 0.8279 & 0.8682 & 0.9913 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0145 & 0.0138 & 0.0114 & 0.0075 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.7605 & 0.8072 & 0.8031 & 0.8926 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0121 & 0.0157 & 0.0129 & 0.0372 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.7150 & 0.7673 & 0.8213 & 0.9898 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0181 & 0.0173 & 0.0155 & 0.0102 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.7085 & 0.7575 & 0.8131 & 0.9865 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0126 & 0.0233 & 0.0173 & 0.0087 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.6547 & 0.6588 & 0.7365 & 0.9930 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0096 & 0.0189 & 0.0145 & 0.0095 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6738 & 0.7073 & 0.7713 & 0.9880 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0128 & 0.0222 & 0.0187 & 0.0134 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.7602 & 0.8097 & 0.8176 & 0.9320 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0107 & 0.0164 & 0.0176 & 0.0182 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.7836 & 0.8291 & 0.8719 & 0.9976 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0135 & 0.0150 & 0.0120 & 0.0032 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.7628 & 0.8165 & 0.8171 & 0.9120 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0171 & 0.0157 & 0.0144 & 0.0204 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.6072 & 0.7274 & 0.7757 & 0.9778 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0110 & 0.0204 & 0.0186 & 0.0180 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.6172 & 0.7242 & 0.7747 & 0.9747 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0080 & 0.0151 & 0.0133 & 0.0166 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.6489 & 0.6513 & 0.7286 & 0.9972 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0148 & 0.0218 & 0.0193 & 0.0057 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.6161 & 0.6719 & 0.7411 & 0.9737 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0128 & 0.0257 & 0.0222 & 0.0137 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.7465 & 0.7909 & 0.7829 & 0.8802 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0189 & 0.0184 & 0.0216 & 0.0319 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.7687 & 0.8231 & 0.8645 & 0.9939 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0140 & 0.0131 & 0.0123 & 0.0060 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.7506 & 0.7918 & 0.7818 & 0.8618 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0131 & 0.0134 & 0.0191 & 0.0474 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.7280 & 0.7678 & 0.8219 & 0.9899 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0186 & 0.0163 & 0.0145 & 0.0101 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.7153 & 0.7542 & 0.8109 & 0.9859 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0131 & 0.0233 & 0.0175 & 0.0113 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.6580 & 0.6578 & 0.7356 & 0.9944 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0146 & 0.0190 & 0.0176 & 0.0093 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.6792 & 0.7119 & 0.7728 & 0.9895 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0119 & 0.0160 & 0.0140 & 0.0101 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.7444 & 0.7873 & 0.7817 & 0.8746 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0099 & 0.0074 & 0.0099 & 0.0213 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.7555 & 0.8092 & 0.8492 & 0.9891 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0105 & 0.0158 & 0.0117 & 0.0066 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.7546 & 0.7961 & 0.7835 & 0.8524 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0129 & 0.0118 & 0.0124 & 0.0276 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.7278 & 0.7616 & 0.8145 & 0.9847 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0123 & 0.0186 & 0.0151 & 0.0090 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.7312 & 0.7576 & 0.8101 & 0.9761 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0191 & 0.0186 & 0.0169 & 0.0202 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.6504 & 0.6705 & 0.7409 & 0.9970 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0157 & 0.0211 & 0.0186 & 0.0061 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6740 & 0.6929 & 0.7559 & 0.9827 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0105 & 0.0157 & 0.0134 & 0.0122 \\
deepwalk\_iterupdate                                & 0.7488 & 0.8353 & 0.8431 & 0.9712 \\
deepwalk\_iterupdate                                & 0.0203 & 0.0224 & 0.0145 & 0.0091 \\
line\_iterupdate                                    & 0.7567 & 0.8342 & 0.8519 & 0.9745 \\
line\_iterupdate                                    & 0.0141 & 0.0181 & 0.0180 & 0.0224 \\
node2vec\_iterupdate                                & 0.7647 & 0.8302 & 0.8448 & 0.9771 \\
node2vec\_iterupdate                                & 0.0147 & 0.0194 & 0.0139 & 0.0139 \\
pca\_iterupdate                                     & 0.6723 & 0.8605 & 0.8630 & 0.9514 \\
pca\_iterupdate                                     & 0.0234 & 0.0106 & 0.0175 & 0.0284 \\
tsvd\_iterupdate                                    & 0.6734 & 0.8302 & 0.8395 & 0.9500 \\
tsvd\_iterupdate                                    & 0.0178 & 0.0529 & 0.0458 & 0.0288 \\
lle\_iterupdate                                     & 0.6566 & 0.9050 & 0.9093 & 0.9796 \\
lle\_iterupdate                                     & 0.0113 & 0.0188 & 0.0156 & 0.0159 \\
isomap\_iterupdate                                  & 0.6703 & 0.8270 & 0.8417 & 0.9622 \\
isomap\_iterupdate                                  & 0.0205 & 0.0223 & 0.0220 & 0.0219
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{fb2 (32)}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.6781 & 0.7205 & 0.6886 & 0.7401 \\
bcgd                                                & 0.0206 & 0.0266 & 0.0260 & 0.0618 \\
deepwalk\_homogeneous\_linear\_projection           & 0.6461 & 0.7019 & 0.6847 & 0.7878 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0188 & 0.0236 & 0.0239 & 0.0354 \\
line\_homogeneous\_linear\_projection               & 0.6573 & 0.7068 & 0.7209 & 0.8907 \\
line\_homogeneous\_linear\_projection               & 0.0144 & 0.0175 & 0.0159 & 0.0266 \\
node2vec\_homogeneous\_linear\_projection           & 0.6551 & 0.7087 & 0.6919 & 0.8032 \\
node2vec\_homogeneous\_linear\_projection           & 0.0147 & 0.0189 & 0.0193 & 0.0296 \\
pca\_homogeneous\_linear\_projection                & 0.5946 & 0.6512 & 0.6720 & 0.8845 \\
pca\_homogeneous\_linear\_projection                & 0.0117 & 0.0137 & 0.0131 & 0.0262 \\
tsvd\_homogeneous\_linear\_projection               & 0.5998 & 0.6697 & 0.6822 & 0.8626 \\
tsvd\_homogeneous\_linear\_projection               & 0.0181 & 0.0256 & 0.0219 & 0.0322 \\
lle\_homogeneous\_linear\_projection                & 0.5498 & 0.5505 & 0.5659 & 0.6573 \\
lle\_homogeneous\_linear\_projection                & 0.0179 & 0.0248 & 0.0218 & 0.0565 \\
isomap\_homogeneous\_linear\_projection             & 0.5764 & 0.6052 & 0.6429 & 0.8610 \\
isomap\_homogeneous\_linear\_projection             & 0.0118 & 0.0117 & 0.0143 & 0.0280 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.6846 & 0.7458 & 0.7298 & 0.8556 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0184 & 0.0253 & 0.0255 & 0.0327 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.6894 & 0.7379 & 0.7561 & 0.9221 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0169 & 0.0182 & 0.0166 & 0.0321 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.6963 & 0.7492 & 0.7335 & 0.8537 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0127 & 0.0154 & 0.0195 & 0.0388 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6386 & 0.6981 & 0.7261 & 0.9224 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0145 & 0.0184 & 0.0202 & 0.0254 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6399 & 0.7150 & 0.7423 & 0.9358 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0115 & 0.0135 & 0.0133 & 0.0204 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5430 & 0.5430 & 0.5757 & 0.7429 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0096 & 0.0145 & 0.0150 & 0.0427 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.6023 & 0.6282 & 0.6699 & 0.8904 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0122 & 0.0159 & 0.0190 & 0.0441 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.6624 & 0.7268 & 0.7150 & 0.8475 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0102 & 0.0157 & 0.0179 & 0.0295 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6617 & 0.7067 & 0.7174 & 0.8730 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0148 & 0.0233 & 0.0262 & 0.0516 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.6107 & 0.6513 & 0.6289 & 0.7100 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0210 & 0.0275 & 0.0240 & 0.0497 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5879 & 0.6375 & 0.6617 & 0.8809 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0088 & 0.0159 & 0.0132 & 0.0240 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5936 & 0.6446 & 0.6650 & 0.8545 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0154 & 0.0253 & 0.0212 & 0.0270 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5485 & 0.5429 & 0.5783 & 0.7667 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0179 & 0.0214 & 0.0207 & 0.0517 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.5828 & 0.5921 & 0.6393 & 0.8581 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0105 & 0.0125 & 0.0134 & 0.0305 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.6842 & 0.7391 & 0.7231 & 0.8420 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0173 & 0.0203 & 0.0217 & 0.0253 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.6939 & 0.7396 & 0.7557 & 0.9082 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0172 & 0.0212 & 0.0231 & 0.0449 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.6880 & 0.7465 & 0.7312 & 0.8499 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0113 & 0.0167 & 0.0197 & 0.0336 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6449 & 0.6922 & 0.7233 & 0.9140 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0122 & 0.0181 & 0.0191 & 0.0258 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6440 & 0.7108 & 0.7406 & 0.9359 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0120 & 0.0157 & 0.0148 & 0.0284 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5441 & 0.5398 & 0.5686 & 0.7063 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0058 & 0.0125 & 0.0104 & 0.0648 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.5982 & 0.6132 & 0.6608 & 0.8903 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0117 & 0.0118 & 0.0154 & 0.0268 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.6773 & 0.7311 & 0.7131 & 0.8310 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0162 & 0.0195 & 0.0183 & 0.0257 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6951 & 0.7428 & 0.7599 & 0.9154 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0167 & 0.0210 & 0.0211 & 0.0293 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.6954 & 0.7507 & 0.7400 & 0.8635 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0164 & 0.0176 & 0.0146 & 0.0260 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6539 & 0.6866 & 0.7240 & 0.9231 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0144 & 0.0161 & 0.0194 & 0.0238 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6652 & 0.7133 & 0.7475 & 0.9376 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0146 & 0.0182 & 0.0191 & 0.0280 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5423 & 0.5450 & 0.5731 & 0.7218 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0092 & 0.0163 & 0.0151 & 0.0588 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.6030 & 0.6155 & 0.6627 & 0.8890 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0108 & 0.0165 & 0.0158 & 0.0255 \\
deepwalk\_iterupdate                                & 0.7116 & 0.8174 & 0.8026 & 0.9324 \\
deepwalk\_iterupdate                                & 0.0213 & 0.0185 & 0.0214 & 0.0242 \\
line\_iterupdate                                    & 0.6840 & 0.7813 & 0.7808 & 0.9406 \\
line\_iterupdate                                    & 0.0118 & 0.0113 & 0.0126 & 0.0279 \\
node2vec\_iterupdate                                & 0.7271 & 0.7894 & 0.7324 & 0.7988 \\
node2vec\_iterupdate                                & 0.0111 & 0.0160 & 0.0232 & 0.0424 \\
pca\_iterupdate                                     & 0.6477 & 0.8134 & 0.8063 & 0.9510 \\
pca\_iterupdate                                     & 0.0188 & 0.0183 & 0.0152 & 0.0221 \\
tsvd\_iterupdate                                    & 0.6381 & 0.7682 & 0.7686 & 0.9510 \\
tsvd\_iterupdate                                    & 0.0134 & 0.0181 & 0.0190 & 0.0299 \\
lle\_iterupdate                                     & 0.5658 & 0.6485 & 0.6717 & 0.9247 \\
lle\_iterupdate                                     & 0.0621 & 0.1567 & 0.2004 & 0.0408 \\
isomap\_iterupdate                                  & 0.6439 & 0.7966 & 0.7990 & 0.9440 \\
isomap\_iterupdate                                  & 0.0156 & 0.0269 & 0.0198 & 0.0191
\end{tabular}
\end{table*}



\begin{table*}[]
\centering
\caption{fb2 (128) }
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.6889 & 0.7524 & 0.7214 & 0.8119 \\
bcgd                                                & 0.0181 & 0.0222 & 0.0214 & 0.0484 \\
deepwalk\_homogeneous\_linear\_projection           & 0.6890 & 0.7559 & 0.7501 & 0.8897 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0145 & 0.0192 & 0.0176 & 0.0282 \\
line\_homogeneous\_linear\_projection               & 0.6589 & 0.7087 & 0.7247 & 0.9031 \\
line\_homogeneous\_linear\_projection               & 0.0151 & 0.0188 & 0.0168 & 0.0228 \\
node2vec\_homogeneous\_linear\_projection           & 0.6899 & 0.7456 & 0.7341 & 0.8609 \\
node2vec\_homogeneous\_linear\_projection           & 0.0148 & 0.0137 & 0.0123 & 0.0320 \\
pca\_homogeneous\_linear\_projection                & 0.5890 & 0.6383 & 0.6645 & 0.8836 \\
pca\_homogeneous\_linear\_projection                & 0.0106 & 0.0163 & 0.0166 & 0.0259 \\
tsvd\_homogeneous\_linear\_projection               & 0.6105 & 0.6817 & 0.6923 & 0.8568 \\
tsvd\_homogeneous\_linear\_projection               & 0.0160 & 0.0200 & 0.0177 & 0.0308 \\
lle\_homogeneous\_linear\_projection                & 0.5403 & 0.5308 & 0.5753 & 0.7604 \\
lle\_homogeneous\_linear\_projection                & 0.0203 & 0.0239 & 0.0202 & 0.0507 \\
isomap\_homogeneous\_linear\_projection             & 0.5841 & 0.6094 & 0.6458 & 0.8572 \\
isomap\_homogeneous\_linear\_projection             & 0.0112 & 0.0122 & 0.0141 & 0.0302 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.6918 & 0.7485 & 0.7439 & 0.8812 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0164 & 0.0177 & 0.0176 & 0.0272 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.7035 & 0.7585 & 0.7725 & 0.9320 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0166 & 0.0152 & 0.0144 & 0.0149 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.6677 & 0.7156 & 0.6993 & 0.8057 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0179 & 0.0188 & 0.0240 & 0.0381 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.6350 & 0.6699 & 0.7065 & 0.9088 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0139 & 0.0232 & 0.0234 & 0.0225 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.6327 & 0.6631 & 0.7084 & 0.9269 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0143 & 0.0154 & 0.0164 & 0.0204 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5427 & 0.5414 & 0.5894 & 0.8078 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0150 & 0.0204 & 0.0210 & 0.0510 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.5879 & 0.5900 & 0.6376 & 0.8563 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0098 & 0.0184 & 0.0146 & 0.0360 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.6829 & 0.7390 & 0.7366 & 0.8866 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0133 & 0.0159 & 0.0192 & 0.0379 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.6884 & 0.7386 & 0.7606 & 0.9331 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0154 & 0.0208 & 0.0171 & 0.0181 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.6765 & 0.7271 & 0.6994 & 0.7818 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0148 & 0.0174 & 0.0159 & 0.0257 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5851 & 0.6314 & 0.6601 & 0.8870 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0110 & 0.0204 & 0.0169 & 0.0239 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5990 & 0.6410 & 0.6669 & 0.8541 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0108 & 0.0143 & 0.0171 & 0.0296 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5375 & 0.5302 & 0.5831 & 0.8173 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0184 & 0.0195 & 0.0164 & 0.0345 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.5827 & 0.5997 & 0.6406 & 0.8583 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0118 & 0.0180 & 0.0171 & 0.0394 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.6867 & 0.7449 & 0.7400 & 0.8849 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0119 & 0.0107 & 0.0128 & 0.0238 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.6945 & 0.7545 & 0.7686 & 0.9204 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0182 & 0.0179 & 0.0173 & 0.0183 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.6659 & 0.7134 & 0.6892 & 0.7706 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0188 & 0.0237 & 0.0220 & 0.0400 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.6383 & 0.6700 & 0.7098 & 0.9159 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0194 & 0.0209 & 0.0231 & 0.0230 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.6359 & 0.6713 & 0.7120 & 0.9248 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0142 & 0.0194 & 0.0179 & 0.0276 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5348 & 0.5321 & 0.5832 & 0.8027 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0186 & 0.0229 & 0.0220 & 0.0635 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.5927 & 0.6010 & 0.6437 & 0.8615 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0125 & 0.0130 & 0.0147 & 0.0360 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.6787 & 0.7274 & 0.7209 & 0.8670 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0108 & 0.0147 & 0.0184 & 0.0350 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.6901 & 0.7444 & 0.7608 & 0.9246 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0177 & 0.0164 & 0.0194 & 0.0232 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.6627 & 0.7038 & 0.6818 & 0.7706 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0163 & 0.0186 & 0.0165 & 0.0298 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.6226 & 0.6384 & 0.6821 & 0.8953 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0117 & 0.0128 & 0.0147 & 0.0323 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.6372 & 0.6593 & 0.6970 & 0.8992 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0178 & 0.0220 & 0.0183 & 0.0206 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5356 & 0.5296 & 0.5814 & 0.7985 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0139 & 0.0187 & 0.0200 & 0.0471 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.5855 & 0.5797 & 0.6201 & 0.8181 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0064 & 0.0113 & 0.0116 & 0.0299 \\
deepwalk\_iterupdate                                & 0.7122 & 0.8197 & 0.8063 & 0.9462 \\
deepwalk\_iterupdate                                & 0.0168 & 0.0150 & 0.0174 & 0.0197 \\
line\_iterupdate                                    & 0.7074 & 0.8142 & 0.8109 & 0.9514 \\
line\_iterupdate                                    & 0.0217 & 0.0233 & 0.0178 & 0.0161 \\
node2vec\_iterupdate                                & 0.7176 & 0.7866 & 0.7259 & 0.7855 \\
node2vec\_iterupdate                                & 0.0111 & 0.0177 & 0.0276 & 0.0611 \\
pca\_iterupdate                                     & 0.6545 & 0.8223 & 0.8174 & 0.9543 \\
pca\_iterupdate                                     & 0.0134 & 0.0167 & 0.0158 & 0.0219 \\
tsvd\_iterupdate                                    & 0.6495 & 0.7876 & 0.7860 & 0.9597 \\
tsvd\_iterupdate                                    & 0.0167 & 0.0176 & 0.0189 & 0.0226 \\
lle\_iterupdate                                     & 0.6691 & 0.8092 & 0.8267 & 0.9469 \\
lle\_iterupdate                                     & 0.0784 & 0.1426 & 0.1128 & 0.0294 \\
isomap\_iterupdate                                  & 0.6614 & 0.8196 & 0.8197 & 0.9466 \\
isomap\_iterupdate                                  & 0.0161 & 0.0231 & 0.0181 & 0.0216
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{sms-a (32)}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.6852 & 0.7250 & 0.7617 & 0.8855 \\
bcgd                 & 0.0027 & 0.0028 & 0.0044 & 0.0340 \\
deepwalk\_iterupdate & 0.6320 & 0.7715 & 0.7845 & 0.9917 \\
deepwalk\_iterupdate & 0.0570 & 0.0158 & 0.0257 & 0.0082 \\
line\_iterupdate     & 0.6001 & 0.6871 & 0.7175 & 0.9952 \\
line\_iterupdate     & 0.0477 & 0.0867 & 0.0842 & 0.0066 \\
node2vec\_iterupdate & 0.7136 & 0.7750 & 0.8048 & 0.9950 \\
node2vec\_iterupdate & 0.0059 & 0.0085 & 0.0068 & 0.0092
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{sms-a (64)}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.6945 & 0.7350 & 0.7770 & 0.9312 \\
bcgd                 & 0.0031 & 0.0037 & 0.0030 & 0.0192 \\
deepwalk\_iterupdate & 0.6228 & 0.7743 & 0.7883 & 0.9914 \\
deepwalk\_iterupdate & 0.0608 & 0.0124 & 0.0232 & 0.0103 \\
line\_iterupdate     & 0.5907 & 0.6743 & 0.7112 & 0.9995 \\
line\_iterupdate     & 0.0450 & 0.0794 & 0.0741 & 0.0014 \\
node2vec\_iterupdate & 0.7164 & 0.7737 & 0.8089 & 1.0000 \\
node2vec\_iterupdate & 0.0052 & 0.0078 & 0.0064 & 0.0000
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{sms-a (128)}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.7017 & 0.7442 & 0.7892 & 0.9714 \\
bcgd                 & 0.0021 & 0.0039 & 0.0025 & 0.0107 \\
deepwalk\_iterupdate & 0.6308 & 0.7760 & 0.7937 & 0.9945 \\
deepwalk\_iterupdate & 0.0619 & 0.0145 & 0.0252 & 0.0062 \\
line\_iterupdate     & 0.5790 & 0.6848 & 0.7195 & 0.9981 \\
line\_iterupdate     & 0.0408 & 0.0600 & 0.0592 & 0.0044 \\
node2vec\_iterupdate & 0.7114 & 0.7574 & 0.7991 & 1.0000 \\
node2vec\_iterupdate & 0.0058 & 0.0069 & 0.0064 & 0.0000
\end{tabular}
\end{table*}


\begin{table}[]
\centering
\caption{HepPH (32) Iterupdate}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.5484 & 0.5681 & 0.6075 & 0.5211 \\
bcgd                 & 0.0023 & 0.0032 & 0.0025 & 0.0219 \\
deepwalk\_iterupdate & 0.5318 & 0.5556 & 0.5665 & 0.8477 \\
deepwalk\_iterupdate & 0.0061 & 0.0069 & 0.0081 & 0.0540 \\
line\_iterupdate     & 0.5422 & 0.5772 & 0.5862 & 0.8809 \\
line\_iterupdate     & 0.0034 & 0.0043 & 0.0039 & 0.0412 \\
node2vec\_iterupdate & 0.5380 & 0.5463 & 0.5528 & 0.2678 \\
node2vec\_iterupdate & 0.0022 & 0.0026 & 0.0029 & 0.0707
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{HepPH (64) Iterupdate}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.5579 & 0.5732 & 0.6170 & 0.5542 \\
bcgd                 & 0.0031 & 0.0031 & 0.0033 & 0.0245 \\
deepwalk\_iterupdate & 0.5345 & 0.5679 & 0.5818 & 0.8623 \\
deepwalk\_iterupdate & 0.0065 & 0.0042 & 0.0051 & 0.0467 \\
line\_iterupdate     & 0.5363 & 0.5677 & 0.5782 & 0.8659 \\
line\_iterupdate     & 0.0036 & 0.0046 & 0.0039 & 0.0421 \\
node2vec\_iterupdate & 0.5431 & 0.5447 & 0.5565 & 0.2812 \\
node2vec\_iterupdate & 0.0022 & 0.0027 & 0.0031 & 0.0846
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{HepPH (128) iterupdate}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.5672 & 0.5771 & 0.6242 & 0.6693 \\
bcgd                 & 0.0042 & 0.0024 & 0.0023 & 0.0630 \\
deepwalk\_iterupdate & 0.5319 & 0.5718 & 0.5886 & 0.8681 \\
deepwalk\_iterupdate & 0.0057 & 0.0027 & 0.0021 & 0.0535 \\
line\_iterupdate     & 0.5327 & 0.5582 & 0.5732 & 0.8435 \\
line\_iterupdate     & 0.0041 & 0.0052 & 0.0035 & 0.0486 \\
node2vec\_iterupdate & 0.5355 & 0.5432 & 0.5423 & 0.1867 \\
node2vec\_iterupdate & 0.0020 & 0.0022 & 0.0022 & 0.0770
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{fb (32) iterupdate}
\label{my-label}
\begin{tabular}{lllll}
method               & acc    & auc    & auprc  & ndcg   \\
bcgd                 & 0.5989 & 0.6431 & 0.6576 & 0.3694 \\
bcgd                 & 0.0021 & 0.0029 & 0.0035 & 0.0257 \\
deepwalk\_iterupdate & 0.7639 & 0.8382 & 0.8312 & 0.9585 \\
deepwalk\_iterupdate & 0.0817 & 0.0645 & 0.0783 & 0.0287 \\
line\_iterupdate     & 0.5958 & 0.6949 & 0.7176 & 0.9887 \\
line\_iterupdate     & 0.0024 & 0.0052 & 0.0025 & 0.0230 \\
node2vec\_iterupdate & 0.7945 & 0.8590 & 0.8590 & 0.9817 \\
node2vec\_iterupdate & 0.0042 & 0.0043 & 0.0050 & 0.0066
\end{tabular}
\end{table}



\begin{table*}[]
\centering
\caption{dblp2 (32) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6986 & 0.7380 & 0.7712 & 0.8568 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0231 & 0.0210 & 0.0270 & 0.0264 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6824 & 0.7163 & 0.7216 & 0.7865 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0241 & 0.0243 & 0.0342 & 0.0439 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6882 & 0.7313 & 0.7545 & 0.8305 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0282 & 0.0279 & 0.0298 & 0.0301 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6853 & 0.7240 & 0.7532 & 0.8300 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0297 & 0.0257 & 0.0307 & 0.0397 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6913 & 0.7253 & 0.7501 & 0.8251 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0244 & 0.0178 & 0.0208 & 0.0244 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6937 & 0.7297 & 0.7556 & 0.8383 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0292 & 0.0298 & 0.0335 & 0.0348 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6855 & 0.7137 & 0.7356 & 0.8094 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0254 & 0.0256 & 0.0343 & 0.0425 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6888 & 0.7192 & 0.7370 & 0.8073 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0270 & 0.0293 & 0.0352 & 0.0448 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6957 & 0.7271 & 0.7573 & 0.8362 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0306 & 0.0330 & 0.0334 & 0.0298 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6899 & 0.7295 & 0.7726 & 0.8636 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0296 & 0.0225 & 0.0210 & 0.0314 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6889 & 0.7240 & 0.7414 & 0.8127 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0328 & 0.0245 & 0.0269 & 0.0323 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.7069 & 0.7458 & 0.7756 & 0.8558 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0236 & 0.0280 & 0.0270 & 0.0315 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6859 & 0.7200 & 0.7480 & 0.8239 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0293 & 0.0263 & 0.0288 & 0.0386 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6348 & 0.7187 & 0.7334 & 0.8089 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0298 & 0.0326 & 0.0353 & 0.0413 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6891 & 0.7309 & 0.7560 & 0.8355 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0213 & 0.0235 & 0.0268 & 0.0352
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{dblp2 (64) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.7163 & 0.7549 & 0.7979 & 0.8942 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0303 & 0.0320 & 0.0313 & 0.0308 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6699 & 0.6862 & 0.6898 & 0.7531 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0318 & 0.0326 & 0.0381 & 0.0505 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.7105 & 0.7447 & 0.7813 & 0.8650 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0240 & 0.0279 & 0.0312 & 0.0380 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.7002 & 0.7382 & 0.7469 & 0.8191 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0274 & 0.0294 & 0.0419 & 0.0466 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6841 & 0.7074 & 0.7238 & 0.7815 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0318 & 0.0327 & 0.0330 & 0.0382 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6866 & 0.7183 & 0.7423 & 0.8169 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0386 & 0.0310 & 0.0302 & 0.0316 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6808 & 0.6965 & 0.7020 & 0.7610 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0385 & 0.0359 & 0.0401 & 0.0503 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6819 & 0.7068 & 0.7156 & 0.7805 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0326 & 0.0295 & 0.0380 & 0.0476 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6768 & 0.6978 & 0.7153 & 0.7819 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0332 & 0.0286 & 0.0347 & 0.0427 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.7007 & 0.7407 & 0.7679 & 0.8519 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0387 & 0.0436 & 0.0440 & 0.0401 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6822 & 0.7035 & 0.7082 & 0.7700 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0308 & 0.0315 & 0.0371 & 0.0505 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.7045 & 0.7518 & 0.7816 & 0.8616 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0281 & 0.0263 & 0.0250 & 0.0223 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6790 & 0.6912 & 0.7046 & 0.7755 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0355 & 0.0360 & 0.0333 & 0.0454 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6696 & 0.6879 & 0.6971 & 0.7629 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0359 & 0.0283 & 0.0375 & 0.0472 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6795 & 0.6981 & 0.7075 & 0.7760 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0326 & 0.0368 & 0.0325 & 0.0379
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{dblp2 (128) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.7125 & 0.7601 & 0.8012 & 0.8950 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0305 & 0.0307 & 0.0306 & 0.0292 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6504 & 0.6544 & 0.6854 & 0.7091 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0319 & 0.0362 & 0.0371 & 0.0684 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.7009 & 0.7394 & 0.7850 & 0.8786 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0254 & 0.0220 & 0.0197 & 0.0252 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6837 & 0.6928 & 0.6967 & 0.7664 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0227 & 0.0247 & 0.0259 & 0.0326 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6578 & 0.6708 & 0.7050 & 0.7275 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0318 & 0.0319 & 0.0283 & 0.0393 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6933 & 0.7144 & 0.7253 & 0.8001 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0274 & 0.0236 & 0.0209 & 0.0274 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6790 & 0.6833 & 0.6886 & 0.7362 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0299 & 0.0244 & 0.0358 & 0.0450 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6417 & 0.6741 & 0.7046 & 0.7356 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0230 & 0.0201 & 0.0244 & 0.0342 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6821 & 0.6950 & 0.7028 & 0.7537 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0336 & 0.0291 & 0.0247 & 0.0299 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6873 & 0.7226 & 0.7435 & 0.8197 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0288 & 0.0287 & 0.0273 & 0.0327 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6884 & 0.7035 & 0.7027 & 0.7607 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0402 & 0.0337 & 0.0441 & 0.0515 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.7034 & 0.7434 & 0.7635 & 0.8370 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0366 & 0.0344 & 0.0332 & 0.0346 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6361 & 0.6515 & 0.6872 & 0.7129 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0221 & 0.0261 & 0.0242 & 0.0411 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6082 & 0.6563 & 0.6927 & 0.7052 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0221 & 0.0338 & 0.0293 & 0.0411 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6505 & 0.6572 & 0.6956 & 0.7129 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0250 & 0.0247 & 0.0258 & 0.0458
\end{tabular}
\end{table*}




\begin{table*}[]
\centering
\caption{dblp3 (32) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.7658 & 0.8166 & 0.8190 & 0.9302 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0099 & 0.0119 & 0.0172 & 0.0288 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.7176 & 0.7615 & 0.7471 & 0.8420 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0138 & 0.0157 & 0.0207 & 0.0433 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.7148 & 0.7763 & 0.7560 & 0.8481 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0125 & 0.0093 & 0.0114 & 0.0324 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.7636 & 0.8146 & 0.8227 & 0.9369 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0105 & 0.0146 & 0.0135 & 0.0202 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.7294 & 0.7814 & 0.7782 & 0.8862 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0142 & 0.0162 & 0.0168 & 0.0282 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.7735 & 0.8295 & 0.8449 & 0.9590 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0198 & 0.0170 & 0.0161 & 0.0162 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.7593 & 0.8119 & 0.8190 & 0.9387 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0111 & 0.0102 & 0.0113 & 0.0129 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.7339 & 0.7862 & 0.7805 & 0.8886 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0157 & 0.0194 & 0.0236 & 0.0284 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.7755 & 0.8295 & 0.8435 & 0.9643 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0144 & 0.0177 & 0.0178 & 0.0230 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.7560 & 0.8117 & 0.8195 & 0.9357 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0151 & 0.0157 & 0.0156 & 0.0193 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.7306 & 0.7811 & 0.7784 & 0.8872 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0148 & 0.0188 & 0.0209 & 0.0311 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.7776 & 0.8322 & 0.8474 & 0.9625 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0181 & 0.0183 & 0.0178 & 0.0166 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.7623 & 0.8161 & 0.8251 & 0.9457 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0130 & 0.0165 & 0.0179 & 0.0182 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6660 & 0.7639 & 0.7568 & 0.8610 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0136 & 0.0219 & 0.0250 & 0.0335 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.7816 & 0.8328 & 0.8476 & 0.9616 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0127 & 0.0090 & 0.0126 & 0.0165
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{dblp3 (64) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.7764 & 0.8295 & 0.8445 & 0.9619 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0109 & 0.0104 & 0.0113 & 0.0189 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.7123 & 0.7522 & 0.7361 & 0.8235 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0155 & 0.0182 & 0.0182 & 0.0369 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.7585 & 0.8121 & 0.8124 & 0.9193 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0094 & 0.0117 & 0.0140 & 0.0211 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.7647 & 0.8151 & 0.8296 & 0.9486 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0103 & 0.0078 & 0.0116 & 0.0175 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.7484 & 0.8025 & 0.8063 & 0.9253 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0137 & 0.0178 & 0.0206 & 0.0293 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.7822 & 0.8366 & 0.8571 & 0.9766 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0138 & 0.0137 & 0.0124 & 0.0128 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.7644 & 0.8178 & 0.8317 & 0.9539 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0113 & 0.0131 & 0.0177 & 0.0161 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.7474 & 0.8000 & 0.8008 & 0.9139 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0088 & 0.0094 & 0.0184 & 0.0363 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.7763 & 0.8360 & 0.8553 & 0.9756 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0161 & 0.0185 & 0.0189 & 0.0191 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.7787 & 0.8301 & 0.8504 & 0.9751 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0144 & 0.0167 & 0.0179 & 0.0148 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.7451 & 0.7907 & 0.7917 & 0.9068 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0138 & 0.0126 & 0.0143 & 0.0184 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.7872 & 0.8367 & 0.8608 & 0.9791 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0164 & 0.0157 & 0.0146 & 0.0129 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.7623 & 0.8160 & 0.8282 & 0.9442 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0085 & 0.0123 & 0.0149 & 0.0197 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.7119 & 0.7811 & 0.7779 & 0.8815 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0179 & 0.0152 & 0.0218 & 0.0477 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.7707 & 0.8266 & 0.8446 & 0.9660 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0113 & 0.0110 & 0.0109 & 0.0210
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{dblp3 (128) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.7908 & 0.8429 & 0.8684 & 0.9834 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0118 & 0.0137 & 0.0119 & 0.0088 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.7402 & 0.7808 & 0.7664 & 0.8496 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0136 & 0.0154 & 0.0207 & 0.0379 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.7864 & 0.8418 & 0.8616 & 0.9708 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0143 & 0.0140 & 0.0147 & 0.0179 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.7502 & 0.7979 & 0.7969 & 0.8980 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0100 & 0.0071 & 0.0117 & 0.0248 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.7540 & 0.8031 & 0.7984 & 0.9017 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0103 & 0.0132 & 0.0181 & 0.0298 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.7603 & 0.8143 & 0.8190 & 0.9277 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0106 & 0.0102 & 0.0137 & 0.0134 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.7392 & 0.7822 & 0.7718 & 0.8605 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0146 & 0.0181 & 0.0227 & 0.0390 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.7425 & 0.7890 & 0.7846 & 0.8849 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0134 & 0.0139 & 0.0187 & 0.0299 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.7560 & 0.8060 & 0.8053 & 0.9109 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0134 & 0.0131 & 0.0157 & 0.0295 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.7513 & 0.8008 & 0.8004 & 0.8997 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0114 & 0.0108 & 0.0169 & 0.0320 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.7461 & 0.7939 & 0.7833 & 0.8707 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0136 & 0.0135 & 0.0174 & 0.0279 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.7738 & 0.8273 & 0.8350 & 0.9356 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0137 & 0.0098 & 0.0122 & 0.0200 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.7338 & 0.7785 & 0.7683 & 0.8566 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0134 & 0.0121 & 0.0195 & 0.0391 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.7302 & 0.7772 & 0.7689 & 0.8654 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0131 & 0.0184 & 0.0198 & 0.0248 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.7491 & 0.7946 & 0.7932 & 0.8914 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0136 & 0.0126 & 0.0186 & 0.0347
\end{tabular}
\end{table*}














\begin{table*}[]
\centering
\caption{fb2 (32) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6809 & 0.7427 & 0.7240 & 0.8507 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0146 & 0.0154 & 0.0219 & 0.0451 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6194 & 0.6520 & 0.6277 & 0.6951 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0145 & 0.0181 & 0.0153 & 0.0553 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6527 & 0.7074 & 0.6844 & 0.7878 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0121 & 0.0171 & 0.0225 & 0.0448 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6366 & 0.6766 & 0.6493 & 0.7258 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0203 & 0.0210 & 0.0197 & 0.0541 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6508 & 0.6947 & 0.6651 & 0.7493 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0167 & 0.0181 & 0.0181 & 0.0469 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6864 & 0.7416 & 0.7268 & 0.8496 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0240 & 0.0243 & 0.0254 & 0.0388 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6285 & 0.6744 & 0.6450 & 0.7310 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0173 & 0.0237 & 0.0193 & 0.0362 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6385 & 0.6816 & 0.6548 & 0.7391 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0142 & 0.0178 & 0.0139 & 0.0323 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6881 & 0.7442 & 0.7280 & 0.8473 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0158 & 0.0169 & 0.0196 & 0.0437 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6198 & 0.6572 & 0.6341 & 0.7176 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0147 & 0.0185 & 0.0195 & 0.0546 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6469 & 0.6891 & 0.6651 & 0.7541 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0113 & 0.0150 & 0.0197 & 0.0476 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.6773 & 0.7446 & 0.7306 & 0.8591 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0105 & 0.0139 & 0.0162 & 0.0333 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6295 & 0.6697 & 0.6395 & 0.7163 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0209 & 0.0283 & 0.0275 & 0.0428 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6380 & 0.6798 & 0.6555 & 0.7457 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0138 & 0.0163 & 0.0208 & 0.0520 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6872 & 0.7402 & 0.7271 & 0.8572 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0114 & 0.0124 & 0.0118 & 0.0263
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{fb2 (64) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6747 & 0.7328 & 0.7199 & 0.8507 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0141 & 0.0173 & 0.0202 & 0.0269 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6128 & 0.6335 & 0.6118 & 0.6637 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0170 & 0.0187 & 0.0209 & 0.0612 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6453 & 0.7018 & 0.6834 & 0.7920 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0221 & 0.0254 & 0.0256 & 0.0432 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6228 & 0.6512 & 0.6266 & 0.6862 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0149 & 0.0203 & 0.0266 & 0.0650 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6366 & 0.6782 & 0.6558 & 0.7431 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0223 & 0.0249 & 0.0245 & 0.0370 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6955 & 0.7549 & 0.7491 & 0.8878 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0109 & 0.0146 & 0.0176 & 0.0354 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6083 & 0.6318 & 0.6057 & 0.6618 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0166 & 0.0168 & 0.0153 & 0.0417 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6316 & 0.6618 & 0.6368 & 0.7018 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0173 & 0.0162 & 0.0148 & 0.0347 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6972 & 0.7559 & 0.7505 & 0.8870 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0131 & 0.0168 & 0.0198 & 0.0320 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6129 & 0.6366 & 0.6099 & 0.6556 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0183 & 0.0180 & 0.0146 & 0.0490 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6304 & 0.6607 & 0.6352 & 0.7068 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0186 & 0.0229 & 0.0213 & 0.0373 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.6867 & 0.7558 & 0.7555 & 0.9055 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0164 & 0.0174 & 0.0143 & 0.0266 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6136 & 0.6395 & 0.6126 & 0.6595 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0170 & 0.0175 & 0.0195 & 0.0519 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6215 & 0.6503 & 0.6239 & 0.6736 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0199 & 0.0238 & 0.0211 & 0.0552 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6858 & 0.7392 & 0.7310 & 0.8672 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0153 & 0.0183 & 0.0200 & 0.0351
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{fb2 (128) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6972 & 0.7595 & 0.7588 & 0.9088 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0159 & 0.0165 & 0.0185 & 0.0232 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6062 & 0.6271 & 0.6049 & 0.6559 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0142 & 0.0161 & 0.0149 & 0.0421 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6878 & 0.7495 & 0.7494 & 0.8905 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0120 & 0.0173 & 0.0163 & 0.0301 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6216 & 0.6523 & 0.6289 & 0.6950 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0150 & 0.0126 & 0.0144 & 0.0403 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6595 & 0.7035 & 0.6870 & 0.7999 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0128 & 0.0158 & 0.0153 & 0.0255 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6910 & 0.7472 & 0.7411 & 0.8818 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0091 & 0.0118 & 0.0130 & 0.0233 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6243 & 0.6492 & 0.6242 & 0.6809 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0179 & 0.0220 & 0.0226 & 0.0618 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6570 & 0.6971 & 0.6761 & 0.7784 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0103 & 0.0102 & 0.0133 & 0.0322 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6899 & 0.7457 & 0.7382 & 0.8777 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0074 & 0.0090 & 0.0098 & 0.0233 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6249 & 0.6503 & 0.6283 & 0.6847 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0171 & 0.0212 & 0.0237 & 0.0607 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6520 & 0.6899 & 0.6692 & 0.7609 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0114 & 0.0158 & 0.0183 & 0.0437 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.6860 & 0.7451 & 0.7499 & 0.9059 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0173 & 0.0190 & 0.0176 & 0.0163 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6241 & 0.6520 & 0.6259 & 0.6815 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0118 & 0.0152 & 0.0152 & 0.0263 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6517 & 0.6902 & 0.6720 & 0.7760 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0163 & 0.0190 & 0.0185 & 0.0305 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6841 & 0.7342 & 0.7239 & 0.8597 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0147 & 0.0173 & 0.0193 & 0.0358
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{CollegeMsg (32) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6520 & 0.6392 & 0.6786 & 0.7838 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0101 & 0.0192 & 0.0077 & 0.0431 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6772 & 0.6545 & 0.6795 & 0.7262 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0145 & 0.0213 & 0.0180 & 0.0507 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6504 & 0.6403 & 0.6750 & 0.7567 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0202 & 0.0326 & 0.0279 & 0.0505 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6729 & 0.6522 & 0.6769 & 0.7193 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0160 & 0.0251 & 0.0146 & 0.0426 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6643 & 0.6424 & 0.6716 & 0.7386 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0124 & 0.0219 & 0.0148 & 0.0479 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6710 & 0.6713 & 0.7017 & 0.7986 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0117 & 0.0149 & 0.0178 & 0.0446 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6693 & 0.6507 & 0.6738 & 0.7096 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0171 & 0.0274 & 0.0174 & 0.0420 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6748 & 0.6646 & 0.6851 & 0.7288 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0135 & 0.0247 & 0.0240 & 0.0550 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6813 & 0.6785 & 0.7053 & 0.7981 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0088 & 0.0150 & 0.0204 & 0.0518 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6796 & 0.6722 & 0.6924 & 0.7434 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0112 & 0.0175 & 0.0176 & 0.0480 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6842 & 0.6758 & 0.6914 & 0.7326 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0122 & 0.0146 & 0.0187 & 0.0620 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.6655 & 0.6626 & 0.6881 & 0.7519 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0126 & 0.0173 & 0.0239 & 0.0670 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6743 & 0.6610 & 0.6809 & 0.7207 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0134 & 0.0238 & 0.0174 & 0.0466 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6803 & 0.6629 & 0.6839 & 0.7368 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0091 & 0.0155 & 0.0170 & 0.0556 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6831 & 0.6774 & 0.6970 & 0.7589 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0089 & 0.0151 & 0.0162 & 0.0462
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{CollegeMsg (64) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6459 & 0.6368 & 0.6741 & 0.7560 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0125 & 0.0164 & 0.0193 & 0.0661 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6578 & 0.6233 & 0.6605 & 0.7153 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0083 & 0.0135 & 0.0194 & 0.0757 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6489 & 0.6433 & 0.6770 & 0.7566 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0090 & 0.0167 & 0.0150 & 0.0467 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6562 & 0.6187 & 0.6615 & 0.7446 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0098 & 0.0166 & 0.0152 & 0.0478 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6572 & 0.6245 & 0.6631 & 0.7234 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0135 & 0.0211 & 0.0248 & 0.0529 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6634 & 0.6595 & 0.7020 & 0.8325 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0068 & 0.0172 & 0.0096 & 0.0342 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6644 & 0.6386 & 0.6700 & 0.7205 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0043 & 0.0165 & 0.0208 & 0.0545 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6629 & 0.6353 & 0.6707 & 0.7387 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0114 & 0.0120 & 0.0184 & 0.0509 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6738 & 0.6745 & 0.7135 & 0.8540 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0080 & 0.0089 & 0.0119 & 0.0321 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6668 & 0.6441 & 0.6763 & 0.7324 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0130 & 0.0198 & 0.0245 & 0.0723 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6666 & 0.6490 & 0.6771 & 0.7308 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0076 & 0.0136 & 0.0149 & 0.0446 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.6720 & 0.6707 & 0.7116 & 0.8344 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0090 & 0.0126 & 0.0151 & 0.0408 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6641 & 0.6431 & 0.6763 & 0.7447 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0097 & 0.0128 & 0.0205 & 0.0630 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6608 & 0.6325 & 0.6657 & 0.7224 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0104 & 0.0156 & 0.0216 & 0.0519 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6780 & 0.6711 & 0.7046 & 0.8083 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0088 & 0.0112 & 0.0158 & 0.0405
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{CollegeMsg (128) non-linear}
\label{my-label}
\begin{tabular}{lllll}
method                                                          & acc    & auc    & auprc  & ndcg   \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.6559 & 0.6577 & 0.6885 & 0.7416 \\
deepwalk\_homogeneous\_nonlinear\_projection\_relu              & 0.0141 & 0.0220 & 0.0246 & 0.0692 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.6632 & 0.6326 & 0.6671 & 0.7135 \\
deepwalk\_homogeneous\_nonlinear\_projection\_sigmoid           & 0.0144 & 0.0230 & 0.0249 & 0.0730 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.6554 & 0.6573 & 0.6959 & 0.7929 \\
deepwalk\_homogeneous\_nonlinear\_projection\_tanh              & 0.0104 & 0.0185 & 0.0135 & 0.0334 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.6551 & 0.6128 & 0.6508 & 0.6890 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_wct       & 0.0085 & 0.0203 & 0.0160 & 0.0544 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.6508 & 0.6022 & 0.6461 & 0.7055 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_wct    & 0.0079 & 0.0104 & 0.0164 & 0.0612 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.6756 & 0.6852 & 0.7253 & 0.8684 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_wct       & 0.0077 & 0.0140 & 0.0123 & 0.0352 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.6530 & 0.6103 & 0.6514 & 0.7112 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_linear    & 0.0046 & 0.0103 & 0.0058 & 0.0326 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.6570 & 0.6157 & 0.6538 & 0.7031 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_linear & 0.0051 & 0.0108 & 0.0136 & 0.0488 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.6808 & 0.6911 & 0.7218 & 0.8364 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_linear    & 0.0076 & 0.0099 & 0.0099 & 0.0385 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.6640 & 0.6359 & 0.6643 & 0.6888 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_avg       & 0.0115 & 0.0176 & 0.0185 & 0.0445 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.6650 & 0.6357 & 0.6686 & 0.7105 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_avg    & 0.0078 & 0.0178 & 0.0189 & 0.0491 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.6721 & 0.6888 & 0.7262 & 0.8733 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_avg       & 0.0105 & 0.0182 & 0.0227 & 0.0488 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.6591 & 0.6208 & 0.6526 & 0.6756 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_relu\_exp       & 0.0100 & 0.0121 & 0.0153 & 0.0380 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.6576 & 0.6175 & 0.6504 & 0.6836 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_sigmoid\_exp    & 0.0086 & 0.0132 & 0.0161 & 0.0508 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.6752 & 0.6564 & 0.6911 & 0.7847 \\
deepwalk\_heterogeneous\_nonlinear\_projection\_tanh\_exp       & 0.0076 & 0.0114 & 0.0134 & 0.0404
\end{tabular}
\end{table*}












\begin{table*}[]
\centering
\caption{NIPS (64) all snap}
\label{my-label}
\begin{tabular}{lllll}
method                                              & acc    & auc    & auprc  & ndcg   \\
bcgd                                                & 0.5170 & 0.5157 & 0.5457 & 0.6118 \\
bcgd                                                & 0.0131 & 0.0193 & 0.0192 & 0.0461 \\
deepwalk\_homogeneous\_linear\_projection           & 0.5536 & 0.5483 & 0.5909 & 0.7892 \\
deepwalk\_homogeneous\_linear\_projection           & 0.0096 & 0.0210 & 0.0229 & 0.0497 \\
line\_homogeneous\_linear\_projection               & 0.5465 & 0.5473 & 0.5794 & 0.7296 \\
line\_homogeneous\_linear\_projection               & 0.0096 & 0.0188 & 0.0187 & 0.0397 \\
node2vec\_homogeneous\_linear\_projection           & 0.5590 & 0.5633 & 0.6123 & 0.7947 \\
node2vec\_homogeneous\_linear\_projection           & 0.0108 & 0.0138 & 0.0151 & 0.0278 \\
pca\_homogeneous\_linear\_projection                & 0.5462 & 0.5446 & 0.5510 & 0.9421 \\
pca\_homogeneous\_linear\_projection                & 0.0127 & 0.0073 & 0.0076 & 0.0268 \\
tsvd\_homogeneous\_linear\_projection               & 0.5360 & 0.5333 & 0.5376 & 0.9623 \\
tsvd\_homogeneous\_linear\_projection               & 0.0146 & 0.0121 & 0.0118 & 0.0261 \\
lle\_homogeneous\_linear\_projection                & 0.5380 & 0.5165 & 0.5488 & 0.7935 \\
lle\_homogeneous\_linear\_projection                & 0.0116 & 0.0181 & 0.0179 & 0.0511 \\
isomap\_homogeneous\_linear\_projection             & 0.5409 & 0.5017 & 0.5389 & 0.8922 \\
isomap\_homogeneous\_linear\_projection             & 0.0307 & 0.0147 & 0.0124 & 0.0337 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.5588 & 0.5532 & 0.6215 & 0.8014 \\
deepwalk\_heterogeneous\_linear\_projection\_wct    & 0.0077 & 0.0218 & 0.0218 & 0.0332 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.5569 & 0.5778 & 0.6093 & 0.8131 \\
line\_heterogeneous\_linear\_projection\_wct        & 0.0101 & 0.0198 & 0.0184 & 0.0375 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.5585 & 0.5581 & 0.6211 & 0.8072 \\
node2vec\_heterogeneous\_linear\_projection\_wct    & 0.0108 & 0.0125 & 0.0171 & 0.0374 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.5370 & 0.5460 & 0.5514 & 0.9626 \\
pca\_heterogeneous\_linear\_projection\_wct         & 0.0112 & 0.0080 & 0.0065 & 0.0197 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.5322 & 0.5272 & 0.5333 & 0.9599 \\
tsvd\_heterogeneous\_linear\_projection\_wct        & 0.0105 & 0.0103 & 0.0097 & 0.0233 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.5237 & 0.5016 & 0.5393 & 0.7190 \\
lle\_heterogeneous\_linear\_projection\_wct         & 0.0062 & 0.0172 & 0.0136 & 0.0486 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.5277 & 0.5195 & 0.5615 & 0.7954 \\
isomap\_heterogeneous\_linear\_projection\_wct      & 0.0053 & 0.0318 & 0.0211 & 0.0289 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.5574 & 0.5497 & 0.6181 & 0.7993 \\
deepwalk\_heterogeneous\_linear\_projection\_avg    & 0.0092 & 0.0165 & 0.0182 & 0.0416 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.5552 & 0.5489 & 0.5865 & 0.8085 \\
line\_heterogeneous\_linear\_projection\_avg        & 0.0118 & 0.0199 & 0.0189 & 0.0490 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.5590 & 0.5557 & 0.6191 & 0.8013 \\
node2vec\_heterogeneous\_linear\_projection\_avg    & 0.0103 & 0.0133 & 0.0151 & 0.0378 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.5320 & 0.5340 & 0.5412 & 0.9439 \\
pca\_heterogeneous\_linear\_projection\_avg         & 0.0102 & 0.0103 & 0.0106 & 0.0435 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.5373 & 0.5338 & 0.5376 & 0.9654 \\
tsvd\_heterogeneous\_linear\_projection\_avg        & 0.0152 & 0.0174 & 0.0151 & 0.0284 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.5253 & 0.5084 & 0.5242 & 0.9283 \\
lle\_heterogeneous\_linear\_projection\_avg         & 0.0070 & 0.0101 & 0.0076 & 0.0341 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.5278 & 0.5531 & 0.5759 & 0.8195 \\
isomap\_heterogeneous\_linear\_projection\_avg      & 0.0084 & 0.0171 & 0.0130 & 0.0311 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.5601 & 0.5565 & 0.6201 & 0.7980 \\
deepwalk\_heterogeneous\_linear\_projection\_linear & 0.0081 & 0.0138 & 0.0153 & 0.0386 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.5572 & 0.5754 & 0.6083 & 0.8200 \\
line\_heterogeneous\_linear\_projection\_linear     & 0.0103 & 0.0185 & 0.0179 & 0.0372 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.5566 & 0.5641 & 0.6233 & 0.7952 \\
node2vec\_heterogeneous\_linear\_projection\_linear & 0.0114 & 0.0214 & 0.0229 & 0.0437 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.5362 & 0.5393 & 0.5465 & 0.9563 \\
pca\_heterogeneous\_linear\_projection\_linear      & 0.0104 & 0.0090 & 0.0079 & 0.0235 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.5363 & 0.5330 & 0.5374 & 0.9445 \\
tsvd\_heterogeneous\_linear\_projection\_linear     & 0.0105 & 0.0117 & 0.0125 & 0.0378 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.5263 & 0.4936 & 0.5397 & 0.6739 \\
lle\_heterogeneous\_linear\_projection\_linear      & 0.0058 & 0.0243 & 0.0170 & 0.0456 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.5315 & 0.5391 & 0.5743 & 0.8198 \\
isomap\_heterogeneous\_linear\_projection\_linear   & 0.0091 & 0.0174 & 0.0148 & 0.0316 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.5622 & 0.5352 & 0.6009 & 0.7674 \\
deepwalk\_heterogeneous\_linear\_projection\_exp    & 0.0124 & 0.0203 & 0.0187 & 0.0348 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.5838 & 0.5896 & 0.6175 & 0.8187 \\
line\_heterogeneous\_linear\_projection\_exp        & 0.0167 & 0.0158 & 0.0169 & 0.0403 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.5718 & 0.5622 & 0.6192 & 0.7849 \\
node2vec\_heterogeneous\_linear\_projection\_exp    & 0.0155 & 0.0189 & 0.0260 & 0.0455 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.5361 & 0.5409 & 0.5472 & 0.9539 \\
pca\_heterogeneous\_linear\_projection\_exp         & 0.0087 & 0.0090 & 0.0070 & 0.0294 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.5370 & 0.5369 & 0.5420 & 0.9559 \\
tsvd\_heterogeneous\_linear\_projection\_exp        & 0.0114 & 0.0141 & 0.0119 & 0.0317 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.5263 & 0.5041 & 0.5581 & 0.6844 \\
lle\_heterogeneous\_linear\_projection\_exp         & 0.0055 & 0.0234 & 0.0197 & 0.0445 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.5367 & 0.5359 & 0.5726 & 0.8209 \\
isomap\_heterogeneous\_linear\_projection\_exp      & 0.0097 & 0.0192 & 0.0138 & 0.0318 \\
deepwalk\_iterupdate                                & 0.5056 & 0.5032 & 0.4879 & 0.3784 \\
deepwalk\_iterupdate                                & 0.0098 & 0.0208 & 0.0171 & 0.0558 \\
line\_iterupdate                                    & 0.5333 & 0.5794 & 0.5484 & 0.4925 \\
line\_iterupdate                                    & 0.0277 & 0.0553 & 0.0365 & 0.1157 \\
node2vec\_iterupdate                                & 0.5283 & 0.5236 & 0.4955 & 0.3700 \\
node2vec\_iterupdate                                & 0.0093 & 0.0215 & 0.0146 & 0.0554 \\
pca\_iterupdate                                     & 0.5072 & 0.4997 & 0.5049 & 0.7532 \\
pca\_iterupdate                                     & 0.0077 & 0.0134 & 0.0064 & 0.0718 \\
tsvd\_iterupdate                                    & 0.5021 & 0.4983 & 0.5039 & 0.7581 \\
tsvd\_iterupdate                                    & 0.0043 & 0.0124 & 0.0054 & 0.0736 \\
lle\_iterupdate                                     & 0.5242 & 0.5480 & 0.5542 & 0.5988 \\
lle\_iterupdate                                     & 0.0306 & 0.0415 & 0.0275 & 0.0833 \\
isomap\_iterupdate                                  & 0.5184 & 0.5108 & 0.5168 & 0.3647 \\
isomap\_iterupdate                                  & 0.0181 & 0.0212 & 0.0115 & 0.1063
\end{tabular}
\end{table*}






